ByteStore: Hybrid Layouts for Main-Memory Column Stores

The performance of main memory column stores highly depends on the scan and lookup operations on the base column layouts. Existing column-stores adopt a homogeneous column layout, leading to sub-optimal performance on real workloads since different columns possess different data characteristics. In this paper, we propose ByteStore, a column store that uses different storage layouts for different columns. We first present a novel data-conscious column layout, PP-VBS (Prefix-Preserving Variable Byte Slice). PP-VBS exploits data skew to accelerate scans without sacrificing lookup performance. Then, we present an experiment-driven column layout advisor to select individual column layouts for a workload. Extensive experiments on real data show that ByteStore outperforms homogeneous storage engines by up to 5.2X.

==> advisor.tex <==


\section{Advisor} \label{sec:advisor}

Based on the design options discussed in Section~\ref{sec:difusion},
in this section,
we present an advisor to compute
the best configuration among 
candidates.
First of all, we require
%which formulates the 
an objective function to analytically quantifies different configurations.
%
%The advisor takes as inputs the basic statistics about the column such as the number of codes in the column $n$, the column width $w$.

%In DIFusion, {\em segments} in a column are possible to be skipped with the index and {\em words} in a segment are possible to be pruned with ByteSlice.
%The objective of DIFusion design is to speed up scan operations.
%%
%Thus, the objective score $\mathcal{S}$ is formulated as the sum of costs used to scan {\em un-skipped segments}, and DIFusion objects to achieve the minimum $\mathcal{S}$ as shown below:
DIFusion aims at accelerating scan operations.
During the scan over data stored in DIFusion layout, segments in a column
are possible to be skipped and 
words in a segment are possible to be early pruned.
Thus, the objective score $\mathcal{S}$ is formulated as the sum of costs for scanning the {\em segments that are not skipped}:
\begin{align}  \label{eq:total_cost}
\text{minimize } \mathcal{S} = & \sum_{i=1}^{N} C_{\text{segment}}(i) \cdot (1 - \rho_{\text{segment}}(i))
\end{align}
%
where $n$ is the total number of codes in the column, $N=\lceil \frac{n}{S/8}\rceil$ represents the total number of segments with SIMD word width $S$,
$\rho_{\text{segment}}(i)$ refers to the probability of skipping the $i$-th segment and 
$C_{\text{segment}}(i)$ is the cost of scanning that segment.
%^{th}
%Without advanced knowledge of the workload,
%we cannot compute the number of {\em un-skipped words} in the $i^{th}$ segment.
%Thus, we estimate $C_{\text{segment}}(i)$ as the expected scan cost $E(C_{\text{segment}})$ oddf each segment, and revise the objective function:
%\begin{align}  \label{eq:total_cost}
%\text{minimize } \mathcal{S} = & E(C_{\text{segment}}) \cdot \sum_{i=1}^{N} (1 - \rho_{\text{segment}}(i))
%\end{align}

In the following, we elaborate each component of the objective function, and analyze the search space of the optimal DIFusion configuration.

%\noindent$\textbf{[}$ {\bf Estimating}  $C_{\text{segment}}(i) \textbf{]}$ 
\stitle{[Estimating $C_{\text{segment}}(i)$]}
%
$C_{\text{segment}}(i)$ represents the cost of scanning words that are not pruned in a segment.
Note that different words in a segment have different probabilities to be pruned, 
thus we estimate
$C_{\text{segment}}(i)$ as its expected value as shown below:
\begin{align}  \label{eq:e_segment_cost}
C_{\text{segment}} = & \sum_{l=1}^{\lceil w/8\rceil} C_{\text{words}}(l) \cdot \rho_{\text{words}}(l)
\end{align}
where $w$ is the code width, $\lceil w/8\rceil$ is the number of words in a segment,
$C_{\text{words}}(l)$ refers to the sum of the cost to process {\em the first $l$ words} in a segment, and 
$\rho_{\text{words}}(l)$ represents the  
probability to {\em early stop processing a segment after $l$ words}.
 
Note that 
the scan of a segment can early stop after $l$ words if 
none of the $S/8$ codes matches the predicate constant
$c$ in the first $l$ words.
The number of bits for comparison in the first $l$ words
is affected by
%
%
%the last $\lceil w/8\rceil-l$ bytes can be pruned in each of the $S/8$ codes in the segment.
%For a code, its $l+1^{th}$ byte cannot be pruned if the {\em data bits} in its first $l$ bytes are identical to those of the predicate literal.
%%{\bf +++ example in background?}
%%
%The number of {\em data bits} in the first $l$ bytes of a code is affected by 
the position 
and the width of the index stored in the segment.
Remember that $k$ and $x$ represent that 
the index occupies $x$ bits in the $k$-th byte of each code in the segment.
%
Then, $\rho_{\text{words}}(l)$ is evaluated as:
\begin{align}  \label{eq:process_word_prob}
\rho_{\text{words}}(l)= 
	\begin{cases} 
 	 \left( 1-(\frac{1}{2})^{8\cdot l} \right)^{S/8}  & 1\leq l< k \\
	\left( 1-(\frac{1}{2})^{8\cdot l-x} \right)^{S/8}  & l\geq k 
   \end{cases}
\end{align}
%
where $8\cdot l-x$ is the number of bits for comparison in the first $l$ bytes of a code for $l\geq k$.
%$1-(\frac{1}{2})^{8\cdot l-x} $ is the probability to prune the last $\lceil w/8\rceil-l$ bytes in a code.

%Since $x$ bits in the $k^{th}$ byte of a code are occupied by the index,
%the number of {\em data bits} in the first $l$ bytes is $8\cdot l$ for $1\leq l< k$ while
 %the number becomes $8\cdot l-x$ for $l\geq k$.
%Thus, $\rho_{\text{words}}(l)$ is calculated as a step-wise function.

%{\color{red}
We obtain $C_{\text{words}}(l)$ through calibration~\cite{xu2016, optimizer13}. %for each $l\in [1, \lceil w/8\rceil]$ 
That is, we consider all the characteristics of the target processor via running calibration experiments on it, and collect the average values.
We take both the cost of data loading/comparison and indexing
extracting/checking into consideration when collecting
$C_{\text{words}}(l)$.
%
%In detail, processing a word includes loading it to SIMD register and comparing it with the predicate.
%If an index vector is stored in it, then index extracting and checking will also be performed.
%%}
%Since the effect of different data and index values on $C_{\text{words}}(l)$ is negligible,
% we measure average cost $C_1(l)$ representing the data loading and comparing cost of $l$ words,
%and average cost $C_2$ representing the cost of extracting and checking an index vector.
%For $1\leq l< k$, we set $C_{\text{words}}(l)$ to $C_1(l)$ while for $l\geq k$, we set $C_{\text{words}}(l)$ to $C_1(l)+C_2$.

%\noindent$\textbf{[}$ {\bf Estimating}  $\rho_{\text{segment}}(i) \textbf{]}$ 
\stitle{[Estimating $\rho_{\text{segment}}(i)$]}
%
$\rho_{\text{segment}}(i)$ is the probability of skipping the $i$-th segment according to the index in DIFusion.
%{\bf +++ modify according to DIFusion part.}
Remember that $\alpha$ is the number of segments 
covered in each indexing target.
%
%We say a segment is covered by an index item if the segment is contained in the target block of the index item.
%
As discussed in Section~\ref{sec:difusion},
 indexing target design in DIFusion follows \cfdesign{}.
Thus, the $i$-th segment is covered by $\beta = \min \{ i-1, \alpha\}$ indexes 
resided in $\beta$ segments from $i-\beta$ to $i-1$.
For example, $\text{Seg}_4$ in left side of Figure~\ref{fig:idx_target}a is covered by indexes resided in $\text{Seg}_2$ and $\text{Seg}_3$.
%
The $i$-th segment can be skipped if at least one of its corresponding $\beta$ indexes is retrieved and indicates to skip its indexing target.
%
An index is retrieved if a) its resident segment is not skipped, and b) the word it lies on is processed.
%
Thus,  $\rho_{\text{segment}}(i)$ is a recursive function, where
$\rho_{\text{segment}}(1)=1$, meaning that the first segment cannot be skipped, and for $i>1$, 
$\rho_{\text{segment}}(i)$ is formulated as:
\begin{align}  \label{eq:process_segment_skip}
\rho_{\text{segment}}(i) = &\nonumber \\
			 \sum_{j=i-\beta}^{i-1} & (1-\rho_{\text{segment}}(j))\cdot (\frac{1}{2})^{8\cdot (k-1)}\cdot \rho_{index}(j)
\end{align}
where $(1-\rho_{\text{segment}}(j))$ represents the probability that the $j$-th segment is  not skipped, 
$\frac{1}{2}^{8\cdot (k-1)}$ is the probability to retrieve the $k$-th word which stores the index, 
and $\rho_{index}(j)$ refers to the probability that the index indicates to skip its indexing target (i.e., the corresponding index checking succeeds).

The skipping condition for the index in DIFusion is similar to that in Column Imprint discussed in Section~\ref{subsec:imprints}.
%{\bf +++ unified with the BackGround, emphasise equal-height histogram. DIFusion discuss this detail?}
Given an index which occupies $x$ bits in each of the $S/8$ codes in a segment, 
its corresponding equal-height histogram contains $x\cdot S/8$ bins.
For a bit in an index, if no values in the indexing target fall in its corresponding bin,
then the bit keeps unset (i.e., 0); otherwise, the bit is set to 1.

\begin{figure}[!h]
	\small \center
	\begin{tabular}{@{}c@{}}
	%\upsmall
	\includegraphics[width=0.99\columnwidth]{figures/index_probability_1} \\
	 (a) For predicates $>, <, \ge, \le$\\
	 %\up
	 \includegraphics[width=0.5\columnwidth]{figures/index_probability_2} \\
	 (b) For predicates $=, \ne$\\
    \end{tabular}
    \caption{Format of Indexes Indicating to Skip Target Segments.}
    %\down
    \label{fig:index_probability}
\end{figure}

%{\bf ++still need a figure here}\\
For {\em predicates} $>$, $<$, $\ge$, $\le$,
%\footnote{
%ByteSlice performs {\tt BETWEEN} by converting it to atomic predicates (i.e.,  $>, <,\ge, \le$) and executes one by one.
%Thus, we consider the skip probabilities of atomic predicates here.
%%, and DIFusion can also support complex predicates in a similar way of ByteSlice.
%}
indexes with successful index checking can be divided into two groups as shown in 
Figure~\ref{fig:index_probability}a, where $c$ is the predicate literal which falls in the bin $b_m$.
%
Indexes in the first group have their last $x\cdot S/8 - m + 1$ bits equal to 0,
which means all values in indexing targets fall in the first $m-1$ bins, and thus each value in target segments satisfies $v<c$.
%
Indexes in the second group have their first $m$ bits equal to 0,
which means all values in indexing targets fall in the last $x\cdot S/8-m$ bins, and thus each value in target segments satisfies $v > c$.
%Thus, in this case, the target segments can be skipped as the comparison result is clear.
%
For indexes from either the first or the second group, 
their corresponding target segments can be skipped since the comparison results between values and $c$ are known.
%Similarly, the execution engine skips examine target segments as the comparison result is clear.
%given a predicate literal which falls in the $b^{th}$ bin,
%the index vector with $x\cdot S/8$ bits will indicate to skip its target if 
%i) all set bits (i.e., bits with 1) lie on the first $b-1$ bits (meaning all target codes less than the predicate literal), or
%ii) all set bits lie on the last $x\cdot S/8-b$ bits (meaning all target codes larger than the predicate literal).
%
Without advanced knowledge of the workload, 
we estimate $\rho_{index}(j)$ using its expected value as shown below:
\begin{align}  \label{eq:index_range_true}
\rho_{index} = &\nonumber \\
			 \sum_{m=1}^{x\cdot S/8}  \frac{1}{x\cdot S/8} \cdot & \left(  (\frac{m-1}{x\cdot S/8})^{\alpha\cdot S/8} + (\frac{x\cdot S/8 -m}{x\cdot S/8})^{\alpha\cdot S/8} \right)
\end{align}
where $\frac{1}{x\cdot S/8}$ represents that the predicate literal has equal probability to fall in any bin of the equal-height histogram,
%the probability that the predicate literal falls in the $b^{th}$ bin of the equal-height histogram,
$(\frac{m-1}{x\cdot S/8})^{\alpha\cdot S/8}$ represents the probability that all the $\alpha\cdot S/8$ codes in the indexing target fall in the first $m-1$ bins of equal-height histogram.

For {\em predicates} $=$, $\neq$, 
given a predicate literal $c$,
only index vectors with the bit $b_m$ unset (see Figure~\ref{fig:index_probability}b) can indicate to skip their target segments.
It is because that unset $b_m$ means no value in indexing targets equals to $c$.
%given a predicate literal which falls in the $b^{th}$ bin,
%the index vector will indicate to skip its target if its $b^{th}$ bit is not set.
%
Thus, we evaluate $\rho_{index}$ as:
\begin{align}  \label{eq:index_point_true}
\rho_{index} =  (\frac{x\cdot S/8 -1}{x\cdot S/8})^{\alpha\cdot S/8}
\end{align}
 
As the workload is unknown, we set $\rho_{index}$ as the average of values calculated 
in Equations~\ref{eq:index_range_true} and~\ref{eq:index_point_true}.
 
%With $E(\rho_{index})$ evaluated in Equations~\ref{eq:index_range_true} and~\ref{eq:index_point_true}, 
%the calculation of $\rho_{\text{segment}}(i) $ in Equation~\ref{eq:process_segment_skip} is revised to:
%
%\begin{align}  \label{eq:process_segment_skip_revise}
%\rho_{\text{segment}}(i) = & \nonumber \\
			%E(\rho_{index}) &~\cdot \frac{1}{2}^{8\cdot (k-1)}\cdot \sum_{j=i-1-\beta}^{i-1} (1-\rho_{\text{segment}}(j))
%\end{align}


%\noindent $\textbf{[}$ {\bf Configuration Search and DIFusion Construction} $\textbf{]}$
\stitle{[Configuration Search]}
With the Equations~\ref{eq:total_cost}, \ref{eq:e_segment_cost} and \ref{eq:process_segment_skip},
the advisor can quantify the performance of different DIFusion configurations.
%
A configuration of DIFusion is a triplet $\langle \alpha, k, x\rangle$, 
and for a column with column width $w$ and the number of segments $N$, 
the options of each component in the configuration is limited:
%
\begin{itemize}
\item $\alpha$: is the number of segments covered in an indexing target, and thus $\alpha< N$
\item $k$: is the position of the word storing index in a segment, and thus $k\leq \lceil w/8\rceil$
\item $x$: is the number of bits occupied by index in one code, and thus $x\leq 8\cdot \lceil w/8\rceil - w$
\end{itemize}
%
%Therefore, the search space to find the optimal configuration is $O(N\cdot \lceil w/8\rceil \cdot (8\cdot \lceil w/8\rceil - w))$.
As the advisor is conducted offline, we can enumerate all configurations\footnote{
From Equations~\ref{eq:index_range_true} and~\ref{eq:index_point_true}, 
$\rho_{index}$ is close to zero with very large $\alpha$, meaning that, the index cannot prune any target codes, while incurring extra index checking cost instead.
We find that in practice, the search space of $\alpha$ can be limited to fewer than 100. 
We retrieve this reduced search range by conducting pre-validation over different columns with various workloads.
}
and choose the one with minimized $\mathcal{S}$ to construct the DIFusion.

With suggested configuration $\langle \alpha, k, x\rangle$ for a column,
its DIFusion is constructed in a similar way to ByteSlice.
The only difference is that, $x\cdot S/8$ bits in the $k$-th word in a segment will be used to store an index and corresponding data bits are push down to the lower-order words.

 %{\bf ++ for experiment: (1) emphasize that if an option combination O1 is better than O2 according to the selection criteria, then the real cost of O1 is smaller than that of O2, for different exp settings}















\iffalse
then there are $\lceil N/(S/8)\rceil$ segments, $\lceil n/8 \rceil$ bytes and $8-n\%8$ vacant bits in each code.
Then the search space for $x$ is $O(8-n\%8)$, 
the search space for $k$ is $\lceil n/8 \rceil$, and for $\alpha$ is $O(\lceil N/(S/8)\rceil)$, 
therefore the the whole search space for the tuneable settings is $O((8-n\%8) * \lceil n/8 \rceil * \lceil N/(S/8)\rceil)$.
In practice, the search space for $\alpha$ is always much smaller than $O(\lceil N/(S/8)\rceil)$ for columns with large $N$, and thus we can enumerate all possible settings to find the optimal one for a given column.

As discussed in Section~\ref{sec:difusion},
to make full use the vacant bits in ByteSlice,
DIFusion stores a secondary index in the vacant bits in a segment.
We store one bit vector in a segment, and the bit vector occupies $x$ bits in the $k^{th}$ byte of all codes in the segment.
Thus one bit vector contains $x * S/8$ bins, where $S$ is the SIMD word width.
The bit vector represents a target block containing $\alpha$ continuous segments from the next segment of the bit vector, 
and thus each segment is represented by $\beta = \alpha$ bit vectors except the first $\alpha$ segments.
%
Therefore, to obtain a good DIFusion for a column,
the appropriate $x$, $k$ and $\alpha$ values must be obtained.
{\bf a foot note to disc special cases?}

To determine the parameter values for $x$, $k$ and $\alpha$, 
we define the selection formula below which models the affect of the parameters on the scan cost with DIFusion.
As mentioned before, the scan cost equals to the sum cost of the scanned segments, and we can use it as 
$$ \mathcal{C} = \sum_{i from 1 to N} \mathcal{C}^{seg}_{i} *(1 - \rho^{seg}_i) $$
where $N$ refers to the total number of segments in the column, 
$\mathcal{C}^{seg}_{i}$ represents the expected cost of processing the $i^{th}$ cost which will be discussed in detail in Section~\ref{sec:advisor_cost_segment}, 
and $\rho^{seg}_i$ is the expected probability that a segment can be skipped as illustrated in Equation~\ref{eq:skip_prob}, and the details to calculate each component of $\rho^{seg}_i$  will be illustrated in Section~\ref{sec:advisor_prob_segment}.


%
In the following, we model the computation formulas to compute $\mathcal{C}^{seg}_{i}$ and (1-$\rho^{seg}_i$).


{\bf ++ for experiment: (1) emphasize that if an option combination O1 is better than O2 according to the selection criteria, then the real cost of O1 is smaller than that of O2, for different exp settings}

\subsection{Expected Scan Cost per Segment $\mathcal{C}^{seg}_{i}$} \label{sec:advisor_cost_segment}
%
Similar to ByteSlice, the scanned cost of a segment is the sum cost of each processed words in it.
If the bit vector occupies $x$ bits in the $k^{th}$ bytes of all codes, 
then for the $j^{th}$ word in the segment, the probability that the word will be processed is:
%
%\usepackage{amsmath}
\begin{align}  \label{eq:process_word_prob}
\rho^{word}_{j+1} = 
	\begin{cases} 
	  1 & j = 1 \\
      1 - (1/2)^{S*j} & 1\le j\leq k \\
      1 - (1/2)^{S/8 * (j * 8 - x)} & j > k 
   \end{cases}
\end{align}
%

And thus the expected of scanning a segment is:
$$\mathcal{C}^{seg}_{i}=\sum_{j from 1 to S/8} \rho^{word}_j * \mathcal{C}^{word}_{i}$$
where $\mathcal{C}^{word}_{i}$ represents the cost to process the $j^{th}$ word in one segment.
As this value varies is affected by uncertain situations, we use benchmarking to get the values of each $\mathcal{C}^{word}_{i}$
for a given column.
{\bf how hebe?}



\subsection{Expected Probability to Scan a Segment $1-\rho^{seg}_i$} \label{sec:advisor_prob_segment}

To expected probability to scan a segment, we need to calcluate the probability that a segment can be skipped.
 As shown in Equation~\ref{eq:skip_prob}, $\rho^{seg}_i$ consists of three components:
$ \rho^{bvskip}$, $ \rho^{byte} $, and $\sum_{\iota=1 to \beta} \rho^{seg}_{j\iota}$.
As we discussed in Section~\ref{sec:difusion_tunable}, 
for a better $\sum_{\iota=1 to \beta} \rho^{seg}_{j\iota}$ with a given $\alpha$,
we should let the bit vector stored in the $i^{th}$ segment represents its following $\alpha$ segments of codes.
And for  $ \rho^{byte} $,  it is the probability of processeing the $k^{th}$ word in the segment if the bit vector is stored in
the $k^{th}$ word, and thus 
$$  \rho^{byte} = (1/2) ^{S*k}$$.

The calculation of $ \rho^{bvskip}$, the probability that a given bit vector indicates its target block can be skipped, 
involves the number of bins in the bit vector and the number of codes in its target block.
%
Let $B$ denote the number of bins in the bit vector and thus $B = x * S/8$ for bit vectors occupying $x$ bits in each code of a segment.
Let $T$ denote the number of codes in the target block and thus $T=\alpha * S/8$ for bit vectors representing $\alpha$ segments in its target block.
%
Remind that, given a bit vector with $B$ bite, it means the domain of the column is divided into $B$ ranges, and each range contains a similar number of values.
Given the value $v$, the probability that $v$ falls in the $m^{th}$ bin is $1/B$ under uniform distribution.
For a predicate literal $c$, asusme that it falls into the $m_{c^{th}}$ bin, then
for predicates $\leq, \le, \geq, \ge$, a bit vector indicates its target block can be skipped is all values in the target block fall in the same side of the  $m_{c^{th}}$ bin.
That is, the target block can be skipped if all target values fall in the first $m_c-1$ bins or all fall in the last $B-m_c$ bins.
Therefore, for predicates $\leq, \le, \geq, \ge$ and given the predicate literal $c$,
the probability of skipping the target block is 
$$ \rho^{bvskip}_{m_c} =  ((m_c - 1) / B)^T + ((B-m_c)/B)^T$$
where $(m_c - 1) / B$ and $(N-m_c)/B$ is the probability that a value falls into the first $m_c-1$ and the last $B-m_c$ bins, respectively.
For predicate $=$, the target block is indicated to be skipped if no value in the target block falls in the $m_{c^{th}}$ bin as the predocate literal does, and thus
$$\rho^{bvskip}_{m_c} =  ((B- 1) / B)^T$$.
%
Since the predicate literal can fall in any of the $B$ bins with equal probability $1/B$, we can derive the expected probability $ \rho^{bvskip}$  of a given bit vector with $B$ bits and $T$ target values:
$$ \rho^{bvskip} = \sum_{m from 1 to B} \rho^{bvskip}_{m} * 1/B$$
\fi





==> algo_numerical.tex <==

\begin{algorithm}[h]
\caption{Prefix Preserving Encoding for Numerical Data}
%\label{algo_categorical}
%\begin{algorithmic}[1]
	\KwIn{
	The frequencies of $n$ distinct values, $q_0, q_1, q_2, ... , q_{n-1}$.
	The number of values in the given column, $N$.
	The height constraint $H$.}
	\KwOut{The minimum cost of the tree.}

	$W[i,i] := 0$, for $0 \le i < n$ \\
	$W[i,j] := \sum_{t=i+1}^{j}q_t$, for $0 \le i < j < n$\\
	\For{$i:=0,1,...,n-1$}
	{	
		$C(i,i,255,h) := 0$, for $0\le h < H$ \\
		\For{$j:=i+1,...,n-1$}
		{
			$min\_height:=\lceil \log_{256}(j-i+1)\rceil$\\
			\If{$min\_height == 1$}
			{
				\For{$h:=0,1,...,H-1$}
				{
					$C(i,j,255,h) := W(i,j)$\\
					$C(i,j,j-i,h) := W(i,j)$\\
					$R(i,j,j-i-1,h) := j$\\
				}
			}
			\Else
			{
				\For{$h:=0,...,min\_height-1$}
				{
					$C(i,j,k,h) := \infty$, for $1\le k < 256$\\
				}
			}
	   	}
	}
	\For{$d:=2,...,n-1$}
	{
		\For{$i:=0,1,...,n-1-d$}
		{
			$j:=i+d$\\
			\For{$h:=1,...,H-1$}
			{
				$C(i,j,1,h) := \infty$\\
				\For{$b:=i+1,...,j$}
				{
					\If{$C(i,b-1,255,h-1)<\infty$ \& $C(b,j,255,h-1)<\infty$}
					{
						$temp:=C(i,b-1,255,h-1)+C(b,j,255,h-1)+W(i,j)$\\
						\If{$temp<C(i,j,1,h)$}
						{
							$C(i,j,1,h):=temp$\\
							$R(i,j,0,h):=b$\\
						}
					}
				}
			}	
			\For{$k:=2,...,\min(255, d-1)$}
			{
				\For{$h:=1,...,H-1$}
				{
					$C(i,j,k,h)=\infty$\\
					$num = (k+1) * (256^h -1) + k$
					\If{$d < num$}
					{
						\For{$b:=R(i, j-1, k-1, h),...,R[i+1, j, k-1, h]$}
						{
							$temp=C(i,b-1,k-1,h)+q_b + W(b,j) + C(b,j,255,h-1)$\\
							\If{$temp < C(i,j,k,h)$}
							{
								$C(i,j,k,h):=temp$\\
								$R(i, j, k-1,h)=b$\\
							}
						}
					}
				}
			}
		}
	}				

\end{algorithm}


==> background.tex <==

\section{Background and Preliminary}\label{sec:background}

%Data is often stored in a compressed form\cite{compressedForm} for many main memory database. Similar to Byteslice, DIFusion is suitable for common compression schemes such as prefix suppression, frame of reference and dictionary encoding\cite{dictionaryEncoding}. With these schemes, native column values are compressed as fix-length order-preserving codes. All data types such as numeric and strings are encoded as unsigned integer codes. For instance, floating point numbers can be multiplied by a specific factor to integers. Strings are encoded by building a sorted dictionary of all distinct strings in that column\cite{distinctString}. 
Data is often stored in a compressed form \cite{blink, fang2010database, farber2012sap, krueger2011fast} for many main memory database. Similar to Byteslice, DIFusion is suitable for common compression schemes such as prefix suppression, frame of reference and dictionary encoding \cite{farber2012sap, krueger2011fast}. With these schemes, native column values are compressed as fix-length order-preserving codes. All data types such as numeric and strings are encoded as unsigned integer codes. For instance, 
%floating point numbers can be multiplied by a specific factor to integers. 
strings are encoded by building a sorted dictionary of all distinct strings in that column~\cite{binnig2009dictionary}. 

In this paper, we focus on the \emph{filter scan} operation in main-memory column store. With a list of $n$ $w$-bit codes as input, a \emph{scan} evaluates a predicate of a range-based comparison, e.g., $=$, $\neq$, $<$, $>$, $\leq$, $\ge$, 
%{\tt BETWEEN}, 
on a single column. Constants in the predicate are in the same domain of the compressed codes. The output of a \emph{scan} is an $n$-bit vector, also called \emph{result bit vector}, which indicates the matching codes that satisfy a predicate. Subsequently, in order to retrieve codes/values from other columns, the result bit vector can be converted to a list of record numbers. A further operation \emph{lookup} will utilize this list of record numbers. A lookup refers to retrieving a code in a column given a record number. Depending the storage layout, a code may have to be reconstructed from multiple memory regions during a lookup. 

\subsection{ByteSlice}

The ByteSlice storage layout regards $S$ contiguous bits in memory as one word. ByteSlice vertically distributes the byte(s) of $w$-bit code across the same bank of $\lceil{w/8}\rceil$ memory words. Figure~\ref{fig:bs} shows an example with $11$-bit column codes. Specially, the column codes are broken down into fixed-length segments, each of which contains $S/8$ codes, where $S$ is the width of a SIMD register. The $S/8$ $w$-bit codes in the segment are then transposed into $l$ = $\lceil{w/8}\rceil$ $S$-bit words, denoted as $W_1$, $W_2$, ..., $W_l$, such that $j$-th byte in $W_i$ equals to the $i$-th byte in the original code $v_j$. 

Scans on ByteSlice formatted data are evaluated segment by segment. Thus, we begin with the discussion of evaluating a GREATER-THAN predicate in a segment. For illustration, consider the following two $17$-bit values $v_1$, $v_2$ and a comparison constant $c$ (with padding 0's underlined):
%\footnote{In this example, ByteSlice has to use 41.2\%(7-bit/17-bit) extra storage as padding zeros for byte-alignment}
\centerline{$v_1 = ($
$10000001$ $11110010$ $1\underline{0000000})_2$}
\centerline{$v_2 = ($
$00001101$ $11001001$ $0\underline{0000000})_2$}
\centerline{ $c = ($
$00100000$	$01001001$ $1\underline{0000000})_2$}
The evaluation is carried out in $\lceil{w/8}\rceil$ iterations, with $j$-th iteration comparing the $j$-th most significant bytes of $v$'s and $c$. For instance, after first iteration ($j=1$), we know:
\centerline{$v_1^{[1]} > c^{[1]}$ and $v_2^{[1]} < c^{[1]}$,}
which allows us to conclude that (1)~$v_1 > c$ and (2)~$v_2 < c$. So, $v_2$ does not satisfy the predicate but $v_1$ does. Therefore, this predicate can early stop and skip the rest iterations. In general, when evaluating the predicate {\tt 'v op c'} ($op={<,  >, \leq, \ge, =, \neq}$), we can early stop after the $j$-th iteration if $v_i \neq c$ for all $v_i$'s. When early stopping occurs in a segment, the scan will proceed to the next segment directly.

Let us illustrate ByteSlice's early stopping with a back-of-the-envelope calculation. Assume the $S/8$ codes of a segment are independent and that the codes and the comparison constant $c$ are random numbers uniformly distributed in the domain of the codes. The probability of a code $v$ matching the constant $c$ at any particular bit position is $1/2$. 
After scanning the most significant $m$ bits of $v$, 
we can conclude the evaluation result for that code 
if any one of those $m$ bits of $v$ does not match the corresponding bit of $c$. The probability of this event is $(1 -– (1/2)^{m})$.  To early stop a segment of $S/8$ codes after examining the codes' most significant $m$ bits, we require the above condition to hold for all $S/8$ codes. Hence, the probability of early stop processing a segment after $m$ bits is:

\centerline{$P_{BS}(m) = (1 - (1/2)^{m})^{S/8}$}

Since ByteSlice processes 1 byte (8 bits) per iteration, so only the probabilities of entries of $m$ that are multiples of 8 are meaningful to be calculated. For example, the probability of early stop at the $W_1$($m$ = $8$) is $0.882$, it means the probability of retrieving $W_2$ is less than $0.12$.

Consider lookup operations in ByteSlice formatted memory data, as each value is sliced into several bytes, one can stitch the bytes back together and remove the padding zeros at the end if needed. For example, looking-up (reconstructing) $v_1$ in Figure~\ref{fig:bs} needs($\ll$ and $\gg$ are left and right shift):
\begin{align*}
v_1 &= \big(BS_1[1] \ll 8 + BS_2[1]\big) \gg 5 \\
	&= \big(01000000_2 \ll 8 + 01100000_2 \big) \gg 5 \\
	%&= (01000000~01100000)_2 \gg 5 \\
	&= (01000000011)_2
\end{align*}
The above example involves two shifts, one addition and two memory reads. Roughly, for each byte involved, it requires a left shift and an addition. A right shift is probably needed at the end in order to remove padding bits.
Lookup on DIFusion formatted memory data involves similar operations, which will 
be illustrated in Section~\ref{sec:exec}.  
%Therefore, if DIFusion still employs padding-right strategy as ByteSlice, the lookup on DIFusion will be the same as on ByteSlice.

\subsection{Column Imprints}\label{subsec:imprints}

A column imprint is a cache conscious secondary indexing structure suitable for both low and high cardinality columns. The main purpose is to quickly identify which blocks of data do not store values that satisfy a range predicate, thereby preventing those blocks from being fetched into the CPU cache for further value comparison. In order to construct a column imprint, the target column is sampled to approximate a histogram of a few (typically $64$ or less) {\em equal-height} bins. Then the entire column is scanned, and for every cacheline of data, a bit vector is created. The bits in the vector correspond to the bins of the histogram. A bit is set if at least one value in the cacheline falls into the corresponding bin.

%\begin{figure}[!h]
%\center
%\includegraphics{figures/imprint}
%\caption{DIFusion}
%\label{fig:Column Imprint}
%\end{figure}

%\begin{figure}[!h]
%	\center
%    \includegraphics[width=0.95\columnwidth]{figures/background_imprint} 
%	\caption{Column Imprint.} \label{fig:Column Imprint}
%\end{figure}
%\begin{figure}[!h]
%	\center
%    \includegraphics[width=0.95\columnwidth]{figures/background_imprint_width} 
%	\caption{Effect of the number of bins in Imprint Vectors.} \label{fig:Imprint_width}
%\end{figure}


\begin{figure}[!h]
	\small \center
	\begin{tabular}{@{}c@{}}
	%\up
	\includegraphics[width=0.95\columnwidth]{figures/background_imprint} \\
	%\down
	 (a) Example: 8-bit Imprint Vectors.\\
	%\upsmall
	 \includegraphics[width=0.9\columnwidth]{figures/background_imprint_width}  \\
	% \down
	 (b) Example: 4-bit Imprint Vectors.\\
    \end{tabular}
    \caption{Column Imprint.} \label{fig:Column Imprint}
    %\down
\end{figure}

Figure~\ref{fig:Column Imprint}a shows a column with $4000$ integer values in the range of $1$ to $1000$. For ease of presentation, assume that each cacheline contains $4$ integer values, and the number of bins is $8$. After uniform sampling, an array of boundaries that partition the domain of the indexed column into equi-height histogram is approximated. Then, by scanning each cacheline, an $8$-bit vector, called \emph{imprint vector}, is created according to the values of the cacheline. For example, the third cacheline consists of $(7, 20, 495, 120)$, among which, $7$, $20$ and $120$ fall into the bin $b_1$ and $495$ falls into the bin $b_4$. As a result, the imprint vector of the first cacheline is ($1001$ $0000$)$_2$. The collection of all the imprint vectors form a column imprint of the target column.

Consequently, while evaluating a query on a column, the execution engine can decide–--in the granularity of a cacheline—-- which parts of the data are irrelevant and safe to be skipped by conducting {\em index checking}. 
%
%remove point query first
%For point queries, consider the instance in Figure~\ref{fig:Column Imprint}a and take {\tt 'V = 200'} as an example. 
%During {\em index checking}, among all bits in an imprint vector,
%%while examining an imprint vector, 
%the execution engine only checks the one corresponds to bin $b_2$ that $200$ falls into. If $b_2$ bit is set, index checking fails and the corresponding cacheline will be retrieved for further process to eliminate false positives; otherwise, index checking succeeds and the cacheline will be skipped to save both memory bandwidth and CPU resource. For instance, in the imprint vector of the cacheline \textcircled{3} in Figure~\ref{fig:Column Imprint}a, the $b_2$ bit is not set, which means this cacheline will be skipped simply. 
%
%Evaluating range queries is more complex.
Take evaluating {\tt 'V $\ge$ 200'} as an example. The first step is to create an empty bit-vector and set the bits that correspond to the bins included in the range $[200, +\infty)$. In this way, we obtain the {\bf query bit-vector} as ($0111$ $1111$)$_2$. 
%In this case, noted that $b_2$ bit should be set, since $200$ falls into bin $b_2$.
%
% The query bit-vector is then checked against every imprint vector. 
Then {\em index checking} is conducted for each imprint vector by bitwise examining 
it against the query bit-vector.
For cacheline \textcircled{1}, the bitwise AND between its imprint vector and query bit-vector is ($0000$ $0000$)$_2$, indicating no common set bits for its imprint vector and the query bit-vector.
It means cacheline \textcircled{1} does not contain any value in the query range, so the execution engine can skip it simply.
%
For cachelines \textcircled{2} and \textcircled{3}, their imprint vectors have common set bits with the query bit-vector.
But the execution engine can still skip cacheline \textcircled{2}.
The reason is that, 
all bins corresponding to the set bits in its imprint vector are fully included in the query range,
meaning that all values in cacheline \textcircled{2} satisfy the query condition.
%, thus the cacheline needs not to be checked at all.
%
From the example we conclude that
%,by checking imprint vectors against
%the query bit-vector,
cachelines can be skipped when: 
%the index checking for an imprint vector is {\bf successful} when:
a) there are no common set bits between the query bit-vector and the imprint vector (e.g., the case of cacheline \textcircled{1}),
or b) all set bits in the imprint vector fall entirely inside the query range (e.g., the case of cacheline \textcircled{2}). 
We say that index checking is 
{\bf successful} when either case 


The number of bits in imprint vectors will affect the probability of successful index checking.
For instance, if we reduce such number of bits in Figure~\ref{fig:Column Imprint}a from 8 to 4,
the imprint vector for cacheline \textcircled{1} becomes ($1000$)$_2$ as shown in Figure~\ref{fig:Column Imprint}b.
In this case, the query bit-vector for predicate {\tt 'V $\ge$ 200'} becomes ($1111$)$_2$, which has common set bits with ($1000$)$_2$.
Thus, with 4-bit imprint vector, cacheline \textcircled{1} needs to be examined to weep out false positives.
Intuitively, {\em index with larger number of bits have higher chance to succeed in index checking}.
%{\color{red}
Column Imprints choose 64 as the number of bits in order
to achieve word alignment for the CPU registers.
In the context of DIFusion, 
we do not have this constraint as wider SIMD registers are available.
In this paper, we use imprints as the secondary index in DIFusion, but with {\em adjustable number of bits}, since it depends on 
the code width of each column. 
%}
%%
%{\bf As a remark, Column Imprint~\cite{} sets 64 as its fixed number of bins in an imprint vector.
%The reason is that......
%However, in DIFusion, no such constraints since we conduct index checking as a by-product of sequential scan}.
%
%
%
%We design the embedded index in DIFusion as a sort of non-dense data skipping structure similar to Column Imprints due to the following two reasons:
%a) it is lightweight to fit within one segment;
%b) it is size-adjustable since the size of valid bits in index is limited by the vacant bits in each segment, 
%which is decided by the code width of the column.



\iffalse
\subsection{Preliminary for DIFusion}
%why we choose imprints
DIFusion inserts secondary index into ByteSlice storage
to enable both early stopping and data skipping 
without any space overhead.
We use $idx_i$ to denote the index contained in Segment $i$.
Basically, $idx_i$ is an $S$-bit bit vector (i.e., word) with $x$-bit occupied
by valid information of $idx_i$'s indexing target.
For the example in Figure~\ref{fig:difusion}b, $x=160$.
We design $idx_i$ as a sort of non-dense data skipping structure similar to Column Imprints due to the following two reasons:
a) it is lightweight to fit within one segment;
b) it is size-adjustable since the size of valid bits in $idx_i$ 
(i.e., the value of $x$) is limited by the vacant bits in each segment, 
which is decided by the code width of the column.

We briefly re-iterate the creation of $idx_i$ next.
Given a column with $w$-bit as the code width,
there are $x=8\cdot \lceil w/8\rceil - w)\times S/8$ valid bits available in $idx_i$.
We first derive a small sample of the column to approximate a histogram of $x$
equal-height bins.
An $x$-bit bit vector is created as index by scanning its indexing target.
A bit is set if at least one value in the target block falls into the corresponding bin.
Finally, these $x$ bits are distributed to a segment according to the design of index (see Section~\ref{sec:difusion}).

Given a scan query, a query bit vector $q$ that has identical valid bits distribution as $idx_i$ could be created (ref. Section~\ref{subsec:imprints}).
Then {\em index checking} could be performed by bitwise intersecting
$q$ and $idx_i$.
The index checking is {\em successful} when the intersecting result
is {\em false}, indicating that $idx_i$'s indexing target could be skipped.
\fi


==> conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
Recently, there is a resurgence of interest in main memory analytic 
databases because of the increasing demand for real-time analytic platforms.
%
Several in-memory storage layouts are invented
to accelerate scans that is a critical operation in columnar.
As a state-of-the-art storage layout, ByteSlice chops
codes into multiple bytes to leverage SIMD for parallel processing and
exploits early-stop capability by high-order bytes comparisons. 
%
However, as column width are usually not multiple of 8-bit, the last-byte of byteSlice is padding with 0's, wasting  memory bandwidth and computation power.
%
To fully leverage these vacant space,
this paper proposes DIFusion, a new storage layout that 
weaves a secondary index into the vacant bits.
%
%
DIFusion enables {\em skip-scan}, a new fast scan that 
inherits the early-stopping capability from ByteSlice
and the same time possesses the data-skipping ability
of index with zero space overhead.
 %
Empirical results report a scan speedup of up to 2.1X, 2.3X, 2.1X, 2.8X on TPC-H, TPC-H Skew, SSB and real workload, respectively.



==> difusion.tex <==
\section{DIFusion} \label{sec:difusion}

\iffalse
{\bf ++assume background already include: 
a) why do we use imprints-similar index in DIFusion?
b) given an x-bit bit vector, how to construct the index by scanning a target
data block.
c) judge if scan by checking the index bit vector with the predicate bit vector

Do we need to repeat what is DIFusion storage and what is skip-scan here?}
\fi

DIFusion weaves the secondary index into the vacant bits 
(i.e., bits originally padded with zeros) to allow data skipping 
during the sequential scan.
As mentioned in the Introduction,
a design option like {\em how to position the index} may affect 
the data skipping probability of the embedded index 
and the early stop capability inherited from ByteSlice
{\em in the opposite way}.
In order to optimize the scan performance on DIFusion,
it is important to dig out all the design options and analyze their
implications.
This section tackles this issue.
As shown in Figure~\ref{fig:framework}, with all the design options available, 
an {\em advisor} is ready to take as input the data column
in standard data type (e.g., 32-bit integer), and generate the {\em best configuration}, where a configuration refers to choices (e.g, parameter setting) of every design option considered.
With the best configuration, the {\em constructor} transforms
the column from raw format to DIFusion.
The details of computing the best configuration in the {\em advisor}
is left to Section~\ref{sec:advisor}.

\begin{figure}[!h]
	\center
	%\up
    \includegraphics[width=0.98\columnwidth]{figures/framework2} 
    %\down
	\caption{DIFusion Construction Framework.} \label{fig:framework}
	%\down
\end{figure}

%argue an index cannot span over multiple words
Similar to scans on ByteSlice, 
scans on DIFusion are performed segment-by-segment,
and the codes in a segment are processed word-by-word.
%We denote an {\em index vector} as a unit component of the index in DIFusion, 
%such as the 160-bit {\em index1} in Figure~\ref{fig:difusion}a.
We argue that an index in DIFusion {\em cannot span multiple words};
otherwise, additional instructions are incurred during the index checking.
As an example in Figure~\ref{fig:difusion}a, 
if 160-bit {\em index1} spans $W_1$ and $W_2$, 
many cycles (e.g., shifting, logical OR) are actually wasted to assemble
{\em index1} from two words into one before checking it against the query bit-vector. 
%{\bf +++is it understandable even with the background section}

With the basic premise above, we discuss the DIFusion design in two steps:
{\bf Step 1)} we regard the design of index {\em within a segment} as a ``black box'', and discuss what the {\em indexing target} of each index should be. 
Specifically, 
the indexing target of {\em index1} is Segment 2 in Figure~\ref{fig:difusion}b.
However, there could be other choices.
{\bf Step 2)} we open the ``black box'' to figure out the specific design of each index.
In Figure~\ref{fig:difusion}a and~\ref{fig:difusion}b, we show that it is possible to position the index in either $W_1$ or $W_2$ of Segment 1. What are the implications? Are there any other considerations in the design of each index?

\begin{figure}[!t]
	\center
    \includegraphics[width=\columnwidth]{figures/indexing_target} \\
%    \up
	\caption{Indexing Target Design.} \label{fig:idx_target}
	\down
\end{figure}

\subsection{Indexing Target Design}\label{subsec:targetdesign}
We call the segment that contains an index as the {\em resident segment} of that index.
Due to the nature of sequential scan,
indexing target of an index should be a batch of continuous codes that appear
{\em after} its resident segment.
Furthermore, we argue that the granularity
of indexing target should be \underline{\em a segment}.
%The major reason is that, words in a segment is the granularity of data loaded
%into SIMD register. The memory access cost can only be saved
%when the whole segment is skipped.
The reason is that, data loading and processing are conducted 
for every $S/8$ codes (i.e., a segment),
which renders skipping partial segment meaningless.

Next, we need to determine which (continuous) segment(s) as the indexing target for each index.
Basically, we illustrate different choices,
and explain why we employ one of them as the fixed choice of this design option.
%other than {\em all other options in the design space}.

\sstitle{\cfdesign{}}
For an index, its indexing target is the
next $\alpha$ segments immediately following its resident segment.

\sstitle{\nrdesign{}}
For an index, its indexing target is
the next $\alpha$ segments that are never covered by other indexes.

Figure~\ref{fig:idx_target}a shows examples about these two designs when $\alpha=2$.
As further elaboration, 
we show the sketch of skip-scan algorithms\footnote{Details of the algorithms will be described in Section~\ref{sec:exec}} based on these two designs in Figure~\ref{fig:idx_target}b.
Regarding the \cfdesign{},
the algorithm scans each segment $\text{\em seg}_i$ word-by-word, 
extracts the index $\text{\em idx}_i$ from $\text{\em seg}_i$,
and performs the index checking for $\text{\em idx}_i$ against the query
bit-vector.
%{\color{red}
If the index checking is successful (c.f. Section~\ref{subsec:imprints}), 
%}
the boolean value $\text{\em flag}$ is set to 1,
and the next $\alpha$ closely-following segments could be skipped
through incrementing $i$ by $\alpha\times \text{\em flag}+1$.
As comparison,
skip-scan over \nrdesign{} incurs extra computation
overhead because
i) it needs to maintain a boolean array (i.e., {\tt skip[]}) to record whether each segment should be skipped or not,
and ii) it needs a conditional statement at the beginning of the loop body, which may incur significant branch mis-prediction penalty.
To justify above analysis, we conduct
experiments on two randomly selected
queries (experimental setting is given
in Section~\ref{sec:exp_design}).
%
Experimental results (c.f. Figure~\ref{fig:exp:CF_NR}) show that \cfdesign{} consistently outperforms \nrdesign{}.
%As a remark, all other choices in the design space have the same extra cost as \nrdesign{}.
Therefore, we fix to use \cfdesign{} in DIFusion
and all the remaining discussions are based on this design.

Note that \cfdesign{} contains a parameter $\alpha$, i.e., the number of segments covered in each indexing target.
We observe that it is non-trivial to determine the value of $\alpha$.
As $\alpha$ increases, more segments are skipped
when the index checking is successful.
However, larger $\alpha$ also reduces the probability of successful index checking.
The reason is that, larger $\alpha$ leads to more values
in the indexing target.
As a result, the index checking is more likely to fail as
the indexing target covers a higher proportion of the domain.
%
%because of the following two observations:
%
%i) When $\alpha$ is larger, more segments are skipped if the index checking is successful. For example, assume any index checking succeeds, 
%the skipped segments account for 50\% of all segments when $\alpha=1$; 
%this percentage increases to 67\% when $\alpha=2$, as for every 
%three segments, the first one is the resident segment, and the next two are the indexing target (ref. \cfdesign{} in Figure~\ref{fig:idx_target}a).
%
%ii) When $\alpha$ is larger, the probability of successful index checking becomes lower, 
%as values in larger indexing target may become less clustered.
%As an extreme case, when $\alpha=N-1$ where $N$ is the total number of segments 
%in a column, index checking in the first segment is very likely to 
%fail as the indexing target (i.e., all remaining $N-1$ segments) covers most domain values. 
%
%{\bf (++should explain what is successful index checking in the background.)}
%
Therefore, in terms of indexing target design, 
$\alpha$ is tunable and should be included in a configuration.


\subsection{Intra-segment Index Design}
After determining the indexing target of each index,
we turn to discuss the detailed design of each index within a segment.

\stitle{[Position of the word storing the index]}
ByteSlice employs {\em Padding-right} strategy since it aims at maximizing 
the early stop probability. With this strategy, the padding zeros are always 
in the last-byte of the $S/8$ codes.
Figure~\ref{fig:difusion}a shows an option of simply replacing those 
padding zeros with the index,
resulting in a 160-bit index scattering over the 2nd-byte of the $S/8$ codes (e.g., $W_2$, $W_4$) in each segment.
%
%However, DIFusion has the chance to prune $W_2$ after scanning $W_1$ since it inherits the early stopping ability of ByteSlice.
%If the pruning happens, the index in $W_2$ can never be retrieved, thus wasting its data skipping ability.
But this option may not always work well for DIFusion.
%
%The early stopping ability inherited from ByteSlice makes DIFusion to have high chance to prune the last bytes of codes,
%and thus DIFusion may fail to retrieve the index vector from segments. %each segment under the {\em Padding-right} option.
%
The reason is that, scan on DIFusion has high
chance to prune the last bytes of codes due to the early stopping ability inherited from ByteSlice. 
In this manner, scan on DIFusion may fail to retrieve
the indexes from segments, wasting their data skipping capability.
%
As an alternative, we could switch to {\em Padding-left} strategy (see Figure~\ref{fig:difusion}b),
which enables us to put the index in the 1st-byte (e.g., $W_1$, $W_3$) in each segment.
%In this way, 
With {\em Padding-left}, the index can definitely be accessed while scanning the segment. %Segment 1.
However, as a side effect, 
%the early stop probability after scanning $W_1$ is reduced.
the early stopping ability will be weakened.
The reason is that, DIFusion can early stop at $W_1$ only when none of the $S/8$ codes in $W_1$ matches the constant $c^{[1]}$ of the predicate;
%and the comparable code width in $W_1$ has been reduced from 8-bit to 3-bit 
%because of the {\em Padding-left} strategy.
%{\color{red}
{\em Padding-left} strategy reduces the number of bits for comparison from 8-bit to 3-bit in each byte of $W_1$ in Figure~\ref{fig:difusion}b;
as a result, the probability of early stop
at $W_1$ is reduced from $(1-(1/2)^\text{\bf 8})^{S/8}$
to $(1-(1/2)^\text{\bf 3})^{S/8}$.
%In the example of Figure~\ref{fig:difusion}b, 
%from 8-bit to 3-bit in .
%{\bf ++need to explain using equations}
%}
%
Basically, we cannot easily determine in which byte shall we arrange the index in a segment.
Given a column with code width $w$,
the index actually could be positioned in any word ranging from 1st word (i.e., word for the most significant byte of codes) 
to $\lceil w/8\rceil$-th word (i.e., word for the least significant byte of codes) by proper bit shifting.
We use $k$ to denote the position of the word in a segment, and it should be included
in a configuration.


\stitle{[Size of the index]}
In above discussion, all vacant bits in a segment are used for the index.
%That is, the size of the index denoted as $x$ equals the number of 
%vacant bits in a segment, i.e.,  $(8\cdot \lceil w/8\rceil - w)\times S/8$.
%That is, in a segment, the number of bits occupied by the index vector (denoted as $x$) in each code
%equals to the number of vacant bits in the code, i.e., $x=8\cdot \lceil w/8\rceil - w$.
That is, the number of bits occupied by index in each code (denoted as $x$) 
{\em equals} the number of vacant bits, i.e., $x=8\cdot \lceil w/8\rceil - w$.
%
Equivalently, the size of result index in each segment is $(8\cdot \lceil w/8\rceil - w)\times S/8$ bits.
However, this choice may not always be optimal,
which can be explained as follows:

i) On the one hand, if the index is not positioned in the $\lceil w/8\rceil$-th word in a segment, 
the bits occupied by index will hurt the early stopping capability of DIFusion.
%Therefore, it is possible to use less than $(8\cdot \lceil w/8\rceil - w)\times S/8$ bits in a segment
Therefore, it is possible to use fewer than
$(8\cdot \lceil w/8\rceil - w)$ bits
as index in each code and leave remaining unused bits to the last byte of each code.
As shown in Figure~\ref{fig:partial_index}, we set $x=2$, which results in
$2\times32=64$-bit index in $W_1$, 
and $3\times 32=96$-bit padding 0's in $W_2$.
%
\begin{figure}[!t]
	\center
	%\up
    \includegraphics[width=0.85\columnwidth]{figures/index_width} \\
    %\down
	\caption{Example of Not Using all Vacant Bits as Index; $w=11$, $S=256$.} \label{fig:partial_index}
	%\down
\end{figure}
%

%ii) On the other hand, index with larger width has higher chance to achieve successful index checking.
%It is because that index vectors with more bits correspond to 
%more fine-grained boundaries of bins in the equal height histogram.
%More fine-grained boundaries may improve the chance to achieve successful index checking (c.f. Section~\ref{subsec:imprints}).

ii) On the other hand, as discussed in Section~\ref{subsec:imprints},
index with larger number of bits are more likely to succeed in index checking.
The main reason is that, index with more bits correspond to more fine-grained bins of the equal-height histogram, which results in higher chance of successful index checking.



%as discussed in the following
%two cases:
%i) If the index vector is positioned in the last-byte of the segment, i.e., $k=\lceil w/8\rceil$, using up all vacant bits as index is always the optimal choice base on Lemma~\ref{lma:index_size}.

%\begin{lemma}\label{lma:index_size}
%Assume two index vectors $\mathcal{I}$ and $\mathcal{I}^{'}$ with width $b$-bit and $b'$-bit, respectively, and $b>b'$.
%If their indexing targets cover the same set of segments, 
%then the skipping probability of $\mathcal{I}$ is not lower than $\mathcal{I}^{'}$.
%there exists predicate bit vector $p$, such that the target could be pruned by $i_1$, but cannot be pruned by $i_2$. Not Vice Verse.
%\end{lemma}
%\begin{proof}
%proof by contradict. to be added.
%\end{proof}

%ii) If the index vector is not positioned in the last-word of the segment, it will hurt the early stopping ability of DIFusion as mentioned in the discussion of selecting $k$.
%Due to this interaction, it is possible to use less than $(8\cdot \lceil w/8\rceil - w)\times S/8$ bits in a segment
%as index and leave remaining vacant bits to the last byte of each code.
%As shown in Figure~\ref{fig:partial_index}, we set $x=2$ and 
%use $2\times32=64$-bit in $W_1$ as an index vector and leave remaining $3\times 32=96$
%vacant bits in $W_2$ unused.

%In general, the value of $x$ could be chosen from the range $[1, 8\cdot \lceil w/8\rceil - w]$.%the set $\{i \times S/8~|~i = 1, 2, ..., 8\cdot \lceil w/8\rceil - w\}$.
%Therefore, $x$ is also tunable and should be included in the configuration.
In general, the value of $x$ ranges from 1 to
($8\cdot \lceil w/8\rceil - w$), and it is non-trivial to decide its value upfront. 
Therefore, $x$ should also be included in a configuration. 

%\subsection{Tagging Index Repeat Number}

%{\bf 
%+++we did not consider the cost of index checking in advisor scoring? why?
%+++talk about the constructor here or at the end of advisor section?
%++where to put minor discussion like ``one segment contains
%at most one bit vecor'', ``bit vectors for a column is homogeneous''}


==> executor.tex <==
\section{Skip-Scan on DIFusion}\label{sec:exec}
%Pseudo-code, example and figure to illustrate each step 
We now describe skip-scans to evaluate comparison predicates over DIFusion 
%($<$, $>$, $\le$, $\ge$, $=$, $\ne$) 
using SIMD instructions.
%The output of such skip-scans is a result bit vector $R$, indicating
%which codes in the column satisfy the predicate.
In general, the column codes are scanned 
segment-by-segment.
Within segment, early stopping capability inherits from ByteSlice is applied.
Furthermore, we have chance to extract the index from the word of $k$-th bytes.
If the index checking against the query bit-vector succeeds, 
the next $\alpha$ segments as indexing target are skipped and the skip-scan proceeds.

\begin{figure}
	\center
    \includegraphics[width=\columnwidth]{figures/skip_scan_algorithm} 
	\caption{Example of Skip-Scan. SIMD word width $S=256$; code width $w=13$; DIFusion configuration $\langle \alpha=2, k=1, x=2\rangle$; word $W_{d1}$ contains an index (i.e., dotted bits).}
	%\down 
	\label{fig:skip_scan_algo}
\end{figure}

We begin with the discussion of evaluating the LESS-THAN predicate `{\tt v < c}' in DIFusion.
%In DIFusion, each scan
%operation processes one segment of codes at a time.
%Inside a segment, codes are processed word-by-word.
%
%To illustrate, we use the example in Figure~\ref{fig:skip_scan_algo} to depict the steps to process the $k^{th}$ word in a segment, 
%which contains an index vector.
For illustration, an example is given in Figure~\ref{fig:skip_scan_algo} where $S=256$ and $w=13$.
The configuration of DIFuison layout is $\langle \alpha=2, k=1, x=2\rangle$,
meaning that for each 13-bit code stored as 2-byte DIFusion layout,
two bits are used as index in the first byte, leaving one bit
for padding 0 in the second byte. 
%the word in the example is the one with index vector (i.e., under-dotted bits in $W_1$).
%
%DIFusion weaves index into data according to the optimal configuration $\langle \alpha, k, x \rangle$.
%
%To conduct skip-scan, the configuration should be given.
% we need to know the configuration first and transfer the comparison value accordingly.
%In the example, 
%index vector in a segment occupies $x=2$ bits in the $1^{st}$ ($k=1$) bytes of each code, and its indexing target covers the closely-following $\alpha=2$ segments.

Given a 13-bit predicate literal $c=(10011001~01001)_2$,
its layout needs to be aligned with data in DIFusion
for the purpose of comparison.
%to compare with codes in DIFusion,
%the layout of $c$ should be consistent with data in DIFusion
%\footnote{
%Two zeros are padded to the 1st byte as $k=1$ and $x=2$.
%The remaining one vacant bit is left in 2nd byte.
%%Inside each byte, putting zero(s) in the left or right end does not affect the process as discussed later.
%}
Thus, $c$ is transformed\footnote{In this example,
$c$ is left-shifted by 2 bits to conduct the transformation;
the concrete operations depend on the value of $k$ and $x$ though. 
} to:
$$ c = (\dotuline{00}100110~0101001\underline{0})_2$$
%
After that, $c$ is broadcasted to $\lceil w/8\rceil$ SIMD words to
get ready for the vectorized comparison (Step \circled{1}).
%
Next, in order to enable data skipping with
index checking, the query bit-vector $\mathcal{BV}_q$
is constructed from the predicate `{\tt v < c}' 
(Step \circled{2}).
%
%At the same time, Step \circled{2} is performed to construct the query bit-vector (i.e., $\mathcal{BV}_q$).
In the example, with $x=2$, we have $x\cdot S/8=64$ (for $S=256$) bits available for index in each
segment;
correspondingly, the column domain is divided into 64 equal-height bins (c.f. Section~\ref{subsec:imprints}).
%
To construct $\mathcal{BV}_q$ in Step \circled{2},
%we:
%\begin{enumerate}[i)]
%\item compute the bin where the literal $c$ falls into
%(i.e., $b_5$),
%\item determine the set bits according to 
%the LESS-THAN nature of the predicate (i.e., $b_1$,
%$b_2$, $\cdots$, $b_5$),
%\item and distribute those bits to different bytes ($x=2$ bits for each byte)
%of the SIMD word (i.e., $\mathcal{BV}_q$).
%\end{enumerate} 
we first compute the bin where the literal $c$ falls into (i.e., $b_5$), and then determine the set bits according to the LESS-THAN nature of the predicate (i.e., $b_1$, $b_2$, $\cdots$, $b_5$),
finally we distribute those bits to different bytes ($x=2$ bits for each byte) of the SIMD word (i.e., $\mathcal{BV}_q$).
%
%to determine the set bits in the query bit-vector (as shown in the dotted rectangle).
%Then, in order to use SIMD instructions, the query bit-vector is broadcasted to a SIMD word
%by allocating $x=2$ bits to each byte.
%For predicate `$V<c$', 
%and then broadcast the predicate bit vector for `$V<c$' to a SIMD word.
% and then broadcast the predicate bit-vector with $x\cdot S/8=64$ (for $S=256$) indexing bits to a SIMD word.
%With $x=2$, the predicate bit-vector $\mathcal{BV}_p$ contains $x\cdot S/8=64$ (for $S=256$) indexing bits, as shown in the dotted rectangle in Step \circled{2}.
%To be consistent with DIFusion, $\mathcal{BV}_p$ is broadcasted to a SIMD word.
%
Step \circled{1} and Step \circled{2} are conducted only once for a given predicate.

With $W_{c1}$, $W_{c2}$ and $\mathcal{BV}_q$ available, 
we proceed to skip-scan the column codes in DIFusion segment-by-segment.
%
%As shown in the example, with $k=1$ and $x=2$,
%the example word $W_1$ contains index vector, and the first 2 bits in each byte are used for index.
As shown in Figure~\ref{fig:skip_scan_algo}, 
$W_{d1}$ is the word for the first byte of $S/8$
codes in a segment.
The first $x=2$ bits of each byte in $W_{d1}$ are occupied by the index.  
To process $W_{d1}$, two operations are performed: 
\begin{enumerate}[i)]
\item Extract index vector $\mathcal{BV}_{\text{\em idx}}$
with the mask $\mathcal{M}_{\text{\em idx}}$ (Step \circled{3})
\item Extract the valid data $W_1$ with the mask $\mathcal{M}_{\text{\em data}}$
(Step \circled{4}), and compare it with corresponding literal word $W_{c1}$.
If the early stop condition is satisfied,
i.e., none of the $S/8$ codes in $W_1$ matches  
the constant in $W_{c1}$,
the remaining word (i.e., $W_{d2}$\footnote{
$W_{d2}$ is not shown in Figure~\ref{fig:skip_scan_algo}; it should be compared with $W_{c2}$ if needed.
}) in the segment can be pruned (Step \circled{5}).
%i) extract the valid data through intersecting $W_{d1}$ with the mask $\mathcal{M}_{\text{\em data}}$, and compare the data with $W_{c1}$ (Step \circled{3}), and 
%ii) extract the index vector through intersecting $W_{d1}$ with the mask $\mathcal{M}_{\text{\em idx}}$, and conduct index checking with $\mathcal{BV}_q$ (Step \circled{4}).
\end{enumerate}
After processing all words in a segment,
the previously obtained index $\mathcal{BV}_{\text{\em idx}}$ are used to
perform index checking (c.f. Section~\ref{subsec:imprints}) against the query bit-vector $\mathcal{BV}_{\text{\em idx}}$ (Step \circled{6}).
%If the early stop condition is satisfied, 
%then the remaining words in the segment can be pruned.
If the checking succeeds, next $\alpha=2$ segments are skipped.
%
%Note that, Steps \circled{3.1} and \circled{4} are only required for words containing index vectors.
%Data comparing in Step \circled{3.2} can be conducted directly for words containing only data bits.

Algorithm~\ref{alg:skipscan} presents the pseudo-code of evaluating the LESS-THAN predicate under DIFusion.
It is self-explanatory and mainly summarizes
what we have discussed in the example above,
so we do not give it a walkthrough here.
It is worth noting that,
we use a if-statement to judge whether a word contains
an index or not (Line~\ref{line:judge}).
In real implementation, we use {\em loop-unrolling} and
instantiate skip-scan functions for distinct $k$ values,
such that the conditional statement is eliminated to avoid
branch mis-prediction penalty.
%Lines~\ref{line:broad_c} and~\ref{line:bvp} conducts Steps \circled{1} and \circled{2},respectively.
%Within a segment processing (Lines~\ref{line:seg_start}-\ref{line:seg_end}),
%data comparison (Steps \circled{3}) is conducted word by word as shown in Lines~\ref{line:word_start}-\ref{line:word_end}.
%Index vector resided in the segment is retrieved in Line~\ref{line:extract_index} 
%and index checking (Steps \circled{4}) is conducted in Line~\ref{line:index_checking}.
%The output of Algorithm~\ref{alg:skipscan} is a result bit vector $R$ whose $i$-th bit is 1 if
%$v_i$ satisfies the predicate or 0 otherwise.
%%
Algorithm~\ref{alg:skipscan}
can be easily modified to handle other comparison
operators (e.g., $>$, $\ge$, $\le$). The details are omitted
for space issue.

%{\bf +++lookup over DIFusion}

%Algorithm 2 shows the pseudo code of PayLess optimization. It
%is self-explanatory and mainly summarizes what we have discussed
%above, so we do not give it a walkthrough here.


\begin{algorithm}
\caption{Skip-Scan on DIFusion ($<$)}
{\fontsize{8}{8}\selectfont
\begin{algorithmic}[1]
\Require{predicate $v < c$, data in DIFusion layout with configuration $\langle \alpha, k, x\rangle$}
\Ensure{result bit vector $R$}
\State Adjust $c$ to align with DIFusion layout        
\For {$j \leftarrow 1 \ldots \lceil \frac{w}{8} \rceil$}
	\State $W_{cj} \leftarrow \texttt{simd\_broadcast}(c^{[j]})$ \Comment{Word with $c$'s $j$-th byte} \label{line:broad_c}
\EndFor 
%\State $\mathcal{BV}_{q}\leftarrow \textsc{bv-less-than}(c, x)$ \Comment{Create the query bit-vector}     \label{line:bvp}
\State Construct the query bit-vector $\mathcal{BV}_{q}$
\State Construct $\mathcal{M}_{\text{\em idx}}$, $\mathcal{M}_{\text{\em data}}$ 
\For {segment $i\leftarrow 0 \ldots N$ with $S/8$ codes $v_{i\cdot S/8+1} \ldots v_{i\cdot S/8+S/8}$}   \label{line:seg_start}
	\State Initialize $\mathcal{M}_{eq} \leftarrow 1^{S}$ and $\mathcal{M}_{lt} \leftarrow 0^{S}$ \Comment{a mask of $S$ 1's / 0's}%means $\underbrace{1\ldots1}_{\text{256 values}}$
%	\State $\mathcal{M}_{lt} \leftarrow 0^{S}$ \Comment{a mask of $S$ 0's}
	\State Create $\mathcal{BV}_{\text{\em idx}} \leftarrow 1^{S}$
	\For {$j \leftarrow 1 \ldots \lceil \frac{w}{8} \rceil$} \label{line:word_start}
		\If {$\texttt{simd\_test\_zero}(\mathcal{M}_{eq})$}
			\State {\bf break}	\Comment{Early stopping}
		\EndIf	
		\State $W_j \leftarrow \texttt{simd\_load}(v_{i\cdot S/8+1}^{[j]} \ldots v_{i\cdot S/8+S/8}^{[j]})$ \Comment{Load the $j$-th bytes}
		\If {$j\equiv k$}	\Comment{Extract index and data at $k$-th byte}	\label{line:judge}
			\State $\mathcal{BV}_{idx} \leftarrow \texttt{simd\_and}(W_j, \mathcal{M}_{\text{\em idx}})$ \label{line:extract_index}
			\State $W_j \leftarrow \texttt{simd\_and}(W_j, \mathcal{M}_{\text{\em data}})$ 
		\EndIf	
		\State $M_{lt} \leftarrow \texttt{simd\_cmplt\_epi8}(W_j, W_{cj})$
		\State $M_{eq} \leftarrow \texttt{simd\_cmpeq\_epi8}(W_j, W_{cj})$
		\State $\mathcal{M}_{lt} \leftarrow \texttt{simd\_or}(M_{lt}, \texttt{simd\_and}(\mathcal{M}_{eq}, M_{lt}))$
		\State $\mathcal{M}_{eq} \leftarrow \texttt{simd\_and}(\mathcal{M}_{eq}, M_{eq})$ 
	\EndFor \label{line:word_end}
	\State $r \leftarrow \texttt{simd\_movemask\_epi8}(\mathcal{M}_{lt})$  \Comment{Condense the mask}
	\State Append $r$ to $R$ \Comment{Append $S/8$ results to final $R$}
	\State $\text{\em flag} \leftarrow \textsc{is-skipped}(\mathcal{BV}_{\text{\em idx}}, \mathcal{BV}_{q}, \alpha)$	\Comment{Index checking}	\label{line:index_checking}
	\State $i \leftarrow \alpha\cdot \text{\em flag} + 1$	\Comment{Skip next $\alpha$ segments} 
\EndFor \label{line:seg_end}
\State \Return $R$
\end{algorithmic}
}
\label{alg:skipscan}
\end{algorithm}
%












\iffalse
Algorithm~\ref{alg:skipscan} presents the pseudo-code
of evaluating the LESS-THAN predicate under DIFusion.
The skip-scan algorithm takes as input a predicate `$v<c$'
and DIFusion data with optimal configuration, 
and outputs a result bit vector $R$ whose $i$-th bit is 1 if
$v_i$ satisfies the predicate or 0 otherwise.
Initially, before broadcasting the constant $c$ to
$\lceil \frac{w}{8} \rceil$ SIMD words,
the algorithm needs to make the layout of $c$
consistent with data in DIFusion layout (Lines~\ref{alg:start1} to~\ref{alg:end1}).
Assume the configuration is $\langle \alpha=2, k=1, x=2\rangle$, step \circled{1} in Figure~\ref{fig:skipscan} illustrates 
an example of adjusting $c$ with code width $w=2$.
Before proceeding to scan data,
the algorithm prepares i) the masks to extract the index 
vector ($\mathcal{M}_{\text{\em idx}}$) and valid data ($\mathcal{M}_{\text{\em data}}$), 
as well as ii) the query bit-vector $\mathcal{BV}_p$.
Algorithm~\ref{alg:bvcreate} describes the process of creating the query bit-vector by distributing the set bits
to different banks of SIMD word. As an example, 
step \circled{2} in Figure~\ref{fig:skipscan}
generates $\mathcal{BV}_p$ based on $c$ when $x=2$.
%$\textsc{bv-less-than}$
Then, the algorithm scans the column codes 
segment-wise, with each segment containing
$S/8$ codes (Lines~\ref{alg:start2} to~\ref{alg:end2}).
This loop body for scanning each column is the same as that for ByteSlice~\cite{} except two differences:
\begin{itemize}
\item While scanning the word where $k$-th bytes are located (i.e., $W_k$),
the algorithm requires to extract the index vector
$\mathcal{BV}_{\text{\em idx}}$ using the mask $\mathcal{M}_{\text{\em idx}}$ (Lines~\ref{alg:start3} to~\ref{alg:end3}).
%If, unfortunately, $W_j$ cannot be accessed 
%due to the early stopping (Lines~\ref{alg:start4} to~\ref{alg:end4})
Here we use a if-statement for easy representation;
in real implementation, we use {\em loop-unrolling} and
instantiate skip-scan functions for distinct $k$ values,
such that the if-statement is eliminated to avoid
branch mis-prediction penalty.
\item After retrieving the index vector,
the algorithm performs indexing checking against 
the query bit-vector (Algorithm~\ref{alg:indexchecking}),
which is similar to the procedures in Column Imprints (ref. Section~\ref{subsec:imprints}).
If the checking succeeds, the algorithm 
skips next $\alpha$ segments (Line~\ref{alg:start5} to~\ref{alg:end5} in Algorithm~\ref{alg:skipscan}).
\end{itemize}
Algorithm~\ref{alg:skipscan}
can be easily modified to handle other comparison
operators (e.g., $\le$). The details are omitted
for space issue.


\begin{figure}[!h]
	\center
   % \includegraphics[width=0.95\columnwidth]{figures/skip_scan} 
	\caption{Example of Skip-scan.} \label{fig:skipscan}
\end{figure}

\begin{algorithm}
\caption{Skip-Scan on DIFusion ($<$)}
{\fontsize{8}{8}\selectfont
\begin{algorithmic}[1]
\Require{predicate $v < c$, data in DIFusion with configuration $\langle \alpha, k, x\rangle$}
\Ensure{result bit vector $R$}
\State Adjust $c$ to align with DIFusion layout \Comment{step \circled{1} in Figure~\ref{fig:skipscan}} \label{alg:start1}
\For {$j \leftarrow 1 \ldots \lceil \frac{w}{8} \rceil$}
	\State $W_{cj} \leftarrow \texttt{simd\_broadcast}(c^{[j]})$ \Comment{Word with $c$'s $j$-th byte}
\EndFor \label{alg:end1}
\State Construct $\mathcal{M}_{\text{\em idx}}$, $\mathcal{M}_{\text{\em data}}$ 
\State $\mathcal{BV}_{p}\leftarrow \textsc{bv-less-than}(c, x)$ \Comment{create query bit-vector}
\For {segment $i\leftarrow 0 \ldots N$ with $S/8$ codes $v_{i\cdot S/8+1} \ldots v_{i\cdot S/8+S/8}$}\label{alg:start2}
	\State $\mathcal{M}_{eq} \leftarrow 1^{S}$ \Comment{a mask of $S$ 1's}%means $\underbrace{1\ldots1}_{\text{256 values}}$
	\State $\mathcal{M}_{lt} \leftarrow 0^{S}$ \Comment{a mask of $S$ 0's}
	\State $\mathcal{BV}_{\text{\em idx}} \leftarrow 1^{S}$
	\For {$j \leftarrow 1 \ldots \lceil \frac{w}{8} \rceil$}
		\If {$\texttt{simd\_test\_zero}(\mathcal{M}_{eq})$}\label{alg:start4}
			\State {\bf break}	\Comment{early stopping}
		\EndIf	\label{alg:end4}
		\State $W_j \leftarrow \texttt{simd\_load}(v_{i\cdot S/8+1}^{[j]} \ldots v_{i\cdot S/8+S/8}^{[j]})$ \Comment{load the $j$-th bytes}
		\If {$j\equiv k$}	\Comment{Extract index and data at $k$-th byte}	\label{alg:start3}
			\State $\mathcal{BV}_{idx} \leftarrow \texttt{simd\_and}(W_j, \mathcal{M}_{\text{\em idx}})$
			\State $W_j \leftarrow \texttt{simd\_and}(W_j, \mathcal{M}_{\text{\em data}})$
		\EndIf	\label{alg:end3}
		\State $M_{lt} \leftarrow \texttt{simd\_cmplt\_epi8}(W_j, W_{cj})$
		\State $M_{eq} \leftarrow \texttt{simd\_cmpeq\_epi8}(W_j, W_{cj})$
		\State $\mathcal{M}_{lt} \leftarrow \texttt{simd\_or}(M_{lt}, \texttt{simd\_and}(\mathcal{M}_{eq}, M_{lt}))$
		\State $\mathcal{M}_{eq} \leftarrow \texttt{simd\_and}(\mathcal{M}_{eq}, M_{eq})$ 
	\EndFor
	\State $r \leftarrow \texttt{simd\_movemask\_epi8}(\mathcal{M}_{lt})$  \Comment{condense the mask}
	\State Append $r$ to $R$ \Comment{Append $S/8$ results to final $R$}
	\State $\text{\em flag} \leftarrow \textsc{is-skipped}(\mathcal{BV}_{\text{\em idx}}, \mathcal{BV}_{p}, \alpha)$	\Comment{index checking}	\label{alg:start5}
	\State $i \leftarrow \alpha\cdot \text{\em flag} + 1$	\Comment{skip next $\alpha$ segments} \label{alg:end5}
\EndFor \label{alg:end2}
\State \Return $R$
\end{algorithmic}
}
\label{alg:skipscan}
\end{algorithm}
%
\begin{algorithm}
\caption{$\textsc{bv-less-than}$ for creating query bit-vector}
{\fontsize{8}{8}\selectfont
\begin{algorithmic}[1]
\Require{query constant $c$, per-code index bit number $x$}
\Ensure{query bit-vector $\mathcal{BV}_{p}$}
\State $\mathcal{BV}_{p}\leftarrow 0^{S}$
\State $b\leftarrow \textsc{getbin}(c)$	\Comment{locate the bin $c$ falls into (ref.~\cite{})}
\For {$i \leftarrow 0\ldots b$}
%\State $\textsc{setbit}(\mathcal{BV}_{p}, 8\cdot \frac{i}{x} + i \mod x)$	\Comment{distribute each set bit to banks}
\State $\textsc{setbit}(\mathcal{BV}_{p}, 8\cdot (\lfloor\frac{i}{x}\rfloor+1) - ((i+1) \mod x) - 1)$	\Comment{distribute each set bit to banks}
\EndFor
\State \Return $\mathcal{BV}_{p}$
\end{algorithmic}
}
\label{alg:bvcreate}
\end{algorithm}
%
\begin{algorithm}
\caption{$\textsc{is-skipped}$ for Index Checking}
{\fontsize{8}{8}\selectfont
\begin{algorithmic}[1]
\Require{query bit-vector $\mathcal{BV}_{p}$, index vector $\mathcal{BV}_{\text{\em idx}}$, indexing target size $\alpha$}
\Ensure{$\text{\em flag}$ indicating whether index checking is successfully}
\State Construct $\mathcal{M}_{\text{\em inner}}$ from $\mathcal{BV}_{p}$ \Comment{the inner-mask}
\If {$\texttt{simd\_and}(\mathcal{BV}_{\text{\em idx}}, \mathcal{BV}_{p})$}	\Comment{index matches query bit vector}
	\If {$\texttt{simd\_and}(\mathcal{BV}_{\text{\em idx}}, \mathcal{M}_{\text{\em inner}})$}
		\State Append $\alpha$ consecutive $1^{S}$ to $R$
		\State \Return {\tt true}
	\EndIf	
	\State \Return {\tt false}
\Else
	\State Append $\alpha$ consecutive $0^{S}$ to $R$	\Comment{append results}
	\State \Return {\tt true}
\EndIf
\end{algorithmic}
}
\label{alg:indexchecking}
\end{algorithm}
\fi

==> experiment.tex <==
\section{Experiment}\label{sec:exp}

\begin{table}[!t]
%\scriptsize
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
Dataset Statistics}
%\down
 % \begin{tabular}{|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|}
 \begin{tabular}{|c|c|c|c|c|c|}
    \hline
	\bf{Dataset} & \bf{Size} & \bf{\#Col} & \bf{Min $w$} & \bf{Max $w$} & \bf{\#Rows}\\
	\hline
	Airtraffic & 27G & 77 & 1 & 14 & 126M\\
	TPC-H Skew 100 & 40G & 26 & 2 & 24 & 600M\\
	TPC-H 100 & 40G & 26 & 2 & 24 & 600M\\
	SSB 100 & 38G & 20 & 3 & 23 & 600M\\
    \hline
  \end{tabular}
  \label{tbl:dataset}
\end{table}

%{\bf ++dataset setting}
%
%---SSB 10G, 100G
%
%---TPC-H, TPC-H Skew 10G, 100G
%
%---real data: air-traffic, 77 columns, just data no query;
%data are updated per month, leading to time-ordered clustered
%sequences. Will reviewer asks, what about those not so clustered data?
%
%
%---range of code width for each dataset
%
%{\bf ++experiment setting}
%
%---single platform or two platforms? just on i7
%
%---Unless stated otherwise, all experiments are run in a single process with a single thread

%
%{\bf ++evaluation}
%
%---\underline{\em important}: multi-threading; more scalable
%
%---\underline{\em important}: is more padding zeros infer 
%better improvement? if yes, why? if no, why?
%this is related to microbenchmark using real data
%
%---How was lookup affected? time dominated by memory access.
%so would not be much slower (ref. section 3.2 in BS); lookup+scan overall performance experiments on, say, TPC-H and SSB?
%
%---real data varying selectivity: on uniform data, should follow the trend of imprints
%
%---skew effect is captured by TPC-H skew?
%
%---Compare two designs: Closely-following vs. No-redundancy

We run our experiments on a personal computer with a 3.40GHz Intel i7-4770 quad-core processor, and 16GB DDR3 memory.
Each core has 32KB L1i cache, 32KB L1d cache and 256KB L2 unified cache.
All cores share an 8MB L3 cache.
The CPU is based on Haswell microarchitecture which supports AVX2 instruction set.
All implementations are done in C++ and compiled using g++ 4.9 with
optimization flag -O3.
We use Intel Performance Counter Monitor \cite{intelpcm} to collect the performance profiles. 
All experiments are run in a single process with a single thread by default.
%We discuss multi-thread experiments in Section \ref{sec:multithread}.

We evaluate our techniques based on TPC-H, TPC-H skew~\cite{tpchskew} (skew factor $zipf=1$), SSB~\cite{o2007star}, and real data. Table~\ref{tbl:dataset} lists the statistics of all datasets.
%
For TPC-H and SSB datasets, to focus only on scans, we follow~\cite{li2014widetable}
to materialize the joins and execute the selection
components of the queries. Queries that involve string similarity comparison {\tt LIKE} are discarded.
%
In TPC-H, 13 queries Q1, Q3, Q4, Q5, Q6, Q8, Q10, Q11, Q12, 
Q14, Q15, Q17, Q19 are eligible.
However, for space reasons, we only selectively present
the results of Q1, Q4, Q6, Q10, Q12, Q15, Q19 on TPC-H 
{\em dbgen} data, Q3, Q5, Q8, Q11, Q14, Q17 on TPC-H skewed
data.
All 13 queries of SSB are eligible.
%
We follow techniques in~\cite{feng2015} to evaluate queries with multiple predicates.
The Airtraffic delay database represents an ever growing
dataset with information about flight delay, landing times,
and other flight statistics\footnote{https://www.percona.com/blog/2009/10/02/analyzing-air-traffic-performance-with-infobright-and-monetdb/}.
In this dataset, 16 out of its 93 columns are excluded because
most of their values are nulls.

\subsection{Impact of Design Options}
\label{sec:exp_design}
To measure the impact
of design options discussed in Section~\ref{sec:difusion} 
on the performance of scan,
we randomly select two queries: i) TPC-H Q1 with predicate {\tt l\_shipdate<=date`1998-11-01'},
and ii) SSB Q2.2 with predicate {\tt p\_brand1=`MFGR\#2221'}.
The attributes {\tt l\_shipdate} and 
{\tt p\_brand1} can be respectively encoded
as {\bf 12-bit} column and {\bf 10-bit} column.
\cfdesign{} and {\em Padding-right} are applied unless otherwise mentioned.
%We use Intel Performance Counter Monitor \cite{intelpcm} to collect the performance profiles. 
%All experiments are run in a single process with a single thread by default.
%We discuss multi-thread experiments in Section \ref{sec:multithread}.

\stitle{[Indexing target]}
As shown in Fig~\ref{fig:exp:CF_NR},
\cfdesign{} outperforms \nrdesign{} consistently,
which echoes our analysis in Section~\ref{subsec:targetdesign}.
With \cfdesign{}, scans in TPC-H Q1 and SSB Q2.2 achieve best performance
when $\alpha$ equals 5 and 2, respectively.
When $\alpha$ gets larger, scans on DIFusion
becomes even slower than that on ByteSlice,
as it is more likely to fail in data skipping, 
and the extra index checking overhead becomes
prominent.

%
\begin{figure}[!h]
 \centering\includegraphics[width=0.9\linewidth]{figures/CF_NR_TPCH}
  \centering\includegraphics[width=0.9\linewidth]{figures/CF_NR_SSB}
 %\vspace{-0.1in}
 %\up
 \caption{Impact of the indexing target design.}
 %\down
 \label{fig:exp:CF_NR}
\end{figure}

\stitle{[Position of the word storing the index]}
As shown in Fig~\ref{fig:exp:padding_direction},
both {\em padding-right} and {\em padding-left} may shine in different queries,
and DIFusion outperforms ByteSlice consistently.

\begin{figure}[!h]
 \centering\includegraphics[width=0.6\linewidth]{figures/padding_direction}
 %\vspace{-0.1in}
 %\up\up
 \caption{Impact of the padding strategy.}
 %\down\down\down
 \label{fig:exp:padding_direction}
\end{figure}

\stitle{[Size of the index]}
With {\em padding-left},
the sizes of the index could vary for columns in TPC-H Q1 and SSB Q2.2, and scans over these columns achieve best performance
when $x$ equals 2 and 3, respectively.


\begin{figure}[!h]
	\small \center
	\begin{tabular}{@{}c@{}c@{}}
	%\up
	\includegraphics[width=0.5\columnwidth]{figures/index_size_TPCH} 
	&
	%\upsmall
	 \includegraphics[width=0.5\columnwidth]{figures/index_size_SSB}  \\
	% \down
    \end{tabular}
    %\up
    \caption{Impact of the index size.}
    %\down\down
     \label{fig:exp:index_size}
    %\down
\end{figure}

\subsection{Skip-Scan Speedup}
%In this experiment, we compare the scan performance 
Figure~\ref{fig:scanspeedup} shows the scan speedup of DIFusion over ByteSlice 
on eligible TPC-H and SSB queries.
We report the average processor cycles per tuple.
From the results,
we observe that DIFusion yields at least 1.4X speedup (TPC-H Q6)
and up to 2.3X (TPC-H Skew Q11).
This is because DIFusion enables both data skipping and early stopping without any space overhead.
%
\begin{figure*}
\center
\includegraphics[width=0.85\linewidth]{figures/scan_speedup}
%\vspace{-2ex}
%\up
\caption{Scan Speed-up over ByteSlice on TPC-H, TPC-H Skew and SSB Queries.}
%\down
\label{fig:scanspeedup}
\end{figure*}

\stitle{[Multi-threading]}
Parallelizing data scans on multi-core is known to be straightforward.
We simply partition data into chunks and assign chunks to the threads.
Figure~\ref{fig:scalability} shows the scan throughput (number of tuples processed per cycle) of TPC-H queries when scans are carried out with different number of threads.
Each thread is pinned to a distinct physical core
in the processor.
From the figure, we can see the throughputs
of both DIFusion and ByteSlice increase when more cores
are used.
These two schemes utilize memory bandwidth effectively
due to their early stopping capability.
Nevertheless, computations on ByteSlice becomes
memory-bound when {\em two} threads are used, 
while computations on DIFusion does not encounter the ``memory-wall'' until {\em four} threads are enabled.
For explanation, we measured the bandwidth utilization
under two schemes.
For example, we found that ByteSlice and DIFusion
used more than 50\% of the available memory bandwidth 
with a single thread.
When two threads are used,
ByteSlice already consumed more than 98\% of the bandwidth
while DIFusion just used about 80\% of the bandwidth.
This explains the scale up behaviors of two schemes as shown in the figure.
Compared to ByteSlice, 
DIFusion exhibits higher throughput with even less memory bandwidth consumption.
The main reason is that, apart from early stop ability,
DIFusion is equipped with index that aims at fetching
relevant (thus less) data, thus alleviating the bandwidth contention especially in the case of multi-threading.
As mentioned in~\cite{li2013bitweaving}, 
effective bandwidth utilization is a key advantage
of sophisticated storage layout schemes 
because one can fully exploit the potentials
of high-end memory subsystems (which the in-memory appliances have) effectively.
From our results,
we see that DIFusion takes this advantage to the next level.

%
\begin{figure*}
\center
\includegraphics[width=\linewidth]{figures/scan_scalability}
%\vspace{-2ex}\
%\up
\caption{Throughput: Varying Number of Cores.}
%\down
\label{fig:scalability}
\end{figure*}

\stitle{[Varying Selectivity]}
To further study the impact of query selectivity on
DIFusion, we use the real data for evaluation, 
and the setting is as follows.
For each of 77 columns, 19 different ranges queries
with varying selectivity are created.
The selectivity starts from 0.05 and increases each time 
by 0.05, until it hits 0.95.
These 19$\times$77=1463 queries are then fired against two layout schemes
(i.e. DIFusion and ByteSlice). 
%So we have 1540 queries in total.
Figure~\ref{fig:selectivity} depicts the factor of improvement
by DIFusion achieved for each query.
A point above 1 is translated as a factor of improvement
over ByteSlice.
From the result, we observe that under any selectivity,
scans over DIFusion can never be slower than that over ByteSlice,
which shows the robustness of our approach.
Furthermore, DIFusion achieves highest speedup (2.8X) for low selectivity queries,
as the index in DIFusion has higher chance to skip more data in this case.
This observation is aligned with the experimental result in~\cite{ColumnImprint} with respect to the impact of query selectivity.


\begin{figure}
\center
\includegraphics[width=0.9\linewidth]{figures/selectivity}
%\vspace{-2ex}
\caption{Improvement over ByteSlice by varying Selectivity.}
%\up
\label{fig:selectivity}
\down
\end{figure}

\subsection{Overall Query Speedup}
%To study the performance of lookup operations under DIFusion 
%layout, we execute projection component apart from selection in TPC-H queries.
As mentioned in the experimental settings,
we follow~\cite{li2014widetable} to materialize joins.
To evaluate the overall performance of DIFusion,
we execute the selection-projection components of the 
TPC-H queries. 
Figure~\ref{fig:whole_speedup} shows the time breakdown of all
eligible queries.
The performance of lookups over DIFusion 
is almost the same as that over ByteSlice.
The reason is that, 
the major overhead of lookups attributes to cache misses 
for reading bytes from different memory regions,
thus rendering the additional masking operation (to erase bits for index) on DIFusion negligible.
Therefore, considering both scans and lookups, 
DIFusion layout yields better performance than ByteSlice
for all tested queries.

%
\begin{figure*}
\center
\includegraphics[width=\linewidth]{figures/whole_speedup}
%\vspace{-2ex}
%\up
\caption{Execution Time Breakdown for TPC-H Queries.}
%\down
\label{fig:whole_speedup}
\end{figure*}


\subsection{Quality of Configuration}\label{subsec:quality}
%
%Experimental results discussed above depict that DIFusion achieves about 
%2X speed-up for scan operations without utilizing extra storage.
%DIFusion storage examined for each column involved in above experiments is
% constructed according to the configuration $\langle \alpha, x, k\rangle$ advised by Equation~\ref{eq:total_cost} in Section~\ref{sec:advisor}, and the layout of indexing targets follows {\em Closely-Following-Design} (Section~\ref{sec:difusion}).
All experiments above show good performance of DIFusion.
In this experiment, we dissect the quality of DIFusion design itself.
Specifically,
we i) first compare the performances of indexing target designs \cfdesign{} and \nrdesign{} (ref. Section~\ref{subsec:targetdesign}), and then ii) examine the quality of the configuration advised by Equation~\ref{eq:total_cost} (ref. Section~\ref{sec:advisor}).
%
To do this, we use the real dataset.
As the column width determines the number of bytes and padding zeros of each column's byte-aligned storage,
we randomly choose one column for each distinct column width among all 77 columns in real dataset, and examine the DIFusion designs using the selected columns.
%
Table~\ref{tab:quality_design}
shows 12 columns with distinct column width\footnote{Columns with $w=8$ are excluded as they are not the target of DIFusion design.} in real dataset.
For each column, we compare the performance of
 {\em CF-Adivsor} versus {\em CF-Enum} and {\em NR-Enum} versus {\em CF-Enum}.
%
With {\em CF-Adivsor}, DIFusion storage is constructed for a column under \cfdesign{} choice with optimal configuration suggested by Equation~\ref{eq:total_cost}.
Its performance over a column is obtained as the average response time of a generated workload $Q$ for that column.
In this experiment, we generate 1000 queries (i.e., $Q$) for each column,
the selectivity of each query is randomly chosen from $[0.05, 0.95]$.
%
As comparison, {\em NR-Enum} and {\em CF-Enum} enumerate all possible configurations $\langle \alpha, x, k\rangle$ for a column,
and for each configuration, two DIFusions are constructed under \cfdesign{} and \nrdesign{}, respectively.
Then, the performance of {\em CF-Enum} is set to the best performance of $Q$ over different DIFusion designs generated under \cfdesign{}. Similarly, we obtain the performance of {\em NR-Enum}.
Values in Table~\ref{tab:quality_design} are calculated as the quality ratio.
%, that is, 
%values in the row {\em CF-Advisor / CF-Enum} are calculated as the performance of {\em CF-Advisor} divided by that of {\em CF-Enum}.
%
From the result in Table~\ref{tab:quality_design}, 
we find that i) indexing target layout \cfdesign{} always outperforms \nrdesign{}, and 
ii) the advisor can find a configuration with performance near to that of the optimal.


\begin{table*}[!htp]
\caption{Quality Test of DIFusion Designs using the Real Dataset.}
%\down\down
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c||@{}c@{}|}
\cline{2-13}
 \multicolumn{1}{c||}{} &  \multicolumn{12}{c||}{Column Width} & \multicolumn{1}{c}{} \\
 \cline{2-14}
 \multicolumn{1}{c||}{} & $w=1$ & $w=2$ & $w=3$ & $w=4$ & $w=5$ & $w=6$ & $w=7$ & $w=9$ & $w=10$ & $w=11$ & $w=13$ & $w=14$ & ~{\bf average}~ \\
 \hline
 \hline
$\frac{CF-Advisor}{CF-Enum}$ & 1  & 1 & 1.07 & 1.09  & 1.08  & 1.11  & 1.09  & 1.08 & 1.09  & 1.10  & 1.08  & 1.09 & 1.07\\
 \hline
 \hline
$\frac{NR-Enum}{CF-Enum}$ & 1.15  & 1.18  & 1.17  & 1.20  & 1.15  & 1.16  & 1.18  & 1.24  & 1.24  & 1.26  & 1.25  & 1.25 & 1.20 \\
\hline
\end{tabular}
\end{center}
\label{tab:quality_design}
\end{table*}%

%\begin{figure*}
%\center
%\includegraphics[width=\linewidth]{figures/tpch-speedup}
%\\(a) Uniform\\
%\includegraphics[width=\linewidth]{figures/tpch-skew1-speedup}
%\\(b) $zipf = 1$\\
%\includegraphics[width=\linewidth]{figures/tpch-skew2-speedup}
%\\(b) $zipf = 2$\\
%\vspace{-2ex}
%\caption{Speed-up over ByteSlice on TPC-H Queries with Uniform Data and Zipfian Data.}
%\label{fig:tpch}
%\end{figure*}



==> introduction.tex <==
\section{Introduction}
In modern main-memory column-stores like SAP HANA~\cite{farber2012sap}, MonetDB~\cite{monetdbx100}, Vectorwise~\cite{zukowski2012vectorwise}, and Oracle Exalytics~\cite{exalytics}, queries are read-mostly, data columns are encoded~\cite{li2013bitweaving, li2015padded} as fixed-length order-preserving {\em codes} for memory efficiency, and their performance goal is to support real-time analytic.
%
%-------------------scan is important, 
Filter-scan, or simply, {\em scan}, is a key operator in main-memory column-stores since ad hoc business intelligence queries frequently use scans over interested columns as base operations.
%There are a plethora of works in main-memory databases on making scans faster.
A scan operation scans a column and returns a result bit vector that indicates which records satisfy a filter predicate.
Recent studies \cite{johnson2008row, li2013bitweaving, feng2015} discuss how to pack multiple codes from the same column into chunks of memory
called {\em words} so as to leverage SIMD to carry out parallel filter evaluation.


%-------------------introduce byteslice
The state-of-the-art storage layout is ByteSlice~\cite{feng2015}, which chops codes into multiple bytes.
%so that scans can be executed very efficiently with minimal overhead. 
Figure~\ref{fig:bs} illustrates how to format thirty-two 11-bit codes ($v_1 \sim v_{32}$) 
into two memory words $W_1$ and $W_2$ in ByteSlice format.
ByteSlice vertically distributes the \emph{bytes} of a $w$-bit code across the same bank of $\lceil w/8 \rceil$ memory words.
In other words, an $S$-bit memory word contains bytes from $S/8$ different codes. These $S/8$ codes form a \textit{segment}.
The magic number 8 comes from the smallest bank width of SIMD multi-operand instructions.
A bank width of 8 bits implies the highest degree of SIMD parallelism, i.e., $S/8$-way.
In this paper, we assume AVX2 \cite{avx512} architecture is used, i.e., $S=256$. 
%We remark that our discussion shall be straightforwardly extended to forthcoming SIMD architectures (e.g., 512-bit AVX-512 \cite{avx512} and Larrabee \cite{larrabee}).

\begin{figure}[!t]
\center
\includegraphics[width=\columnwidth]{figures/bs_single}
\caption{ByteSlice.}
%\up
\label{fig:bs}
\down
\end{figure}
%
In Figure~\ref{fig:bs},
the first bytes of $v_1 \sim v_{32}$ are packed into the banks of $W_1$.
The remaining 3 bits are packed into the banks of $W_2$ in a way similar to $W_1$, with {\em padding zeros} at the end.
%In contrast to the folklore of padding 0's at the front,
%padding at the end can maximize the early stopping probability during scan.
The next segment of 32 codes ($v_{33} \sim v_{64}$) are formatted in the same way into words $W_3$ and $W_4$.
Words that contain the $i$-th bytes of codes are stored in a contiguous memory region as one ByteSlice.
In Figure~\ref{fig:bs}, $W_1$ and $W_3$ are stored in ByteSlice $BS_1$
whereas $W_2$ and $W_4$ are stored in ByteSlice $BS_2$.

%-------------------early stop of bs
Scans on ByteSlice are efficient because of \emph{early stopping}.
We use the notation $v^{[i]}$ to denote the $i$-th byte of value $v$. 
For example, in Figure~\ref{fig:bs}, $v_{32}^{[1]} = (00110000)_2$
and $v_{32}^{[2]} = (110~\underline{00000})_2$.
So, assuming the {\tt WHERE} predicate is $v = c$ 
but no bytes in word $W_1$ match $c^{[1]}$,
i.e., $v_i^{[1]} \neq c^{[1]}$, for $i=1$ to $32$.
Then, 
after processing $W_1$,
the scan operation can early stop, i.e., skip word $W_2$ and proceed to process $W_3$ instead.

\begin{figure*}[t]
\center
\includegraphics[width=.87\linewidth]{figures/difusion_intro}
\caption{DIFusion.}
\up
\label{fig:difusion}
\down
\end{figure*}
%
%\begin{figure}[!h]
%\center
%\includegraphics[width=\columnwidth]{figures/intro_}
%\caption{Comparison of DIFusion and ByteSlice.}
%\up
%\label{fig:difusion}
%\down
%\end{figure}
%----------------problem of wasting padding zeros
As ByteSlice chops codes into multiple bytes,
it is inevitable to use zeros to pad up with the 8-bit SIMD soft boundaries.
%the codes such that the byte-alignment is achieved.
For the 11-bit codes in Figure~\ref{fig:bs}, 
%we have to use 45\% extra storage as padding zeros for byte-alignment.
65.5\% bits are padding zeros for byte-alignment in ByteSlice $BS_2$.
%As another example, {\tt l\_shipmode} column in TPC-H is encoded in 3-bit,
%resulting in 167\% extra storage for padding zeros.
In TPC-H and SSB data stored as ByteSlice,
96\% and 90\% of their columns have padding zeros, respectively.
Under ByteSlice, padding zeros accounts for 31\% and 37\% of the whole storage in TPC-H and SSB data, respectively~\cite{feng2015}.
These unexploited zeros lead to wasting resources in two aspects:
i) Memory bandwidth is under-utilized while loading memory word with padding zeros (e.g., $W_2$ in Figure~\ref{fig:bs})
from RAM to SIMD register.
This is wasteful, especially in the era of growing imbalance between CPU clock-speed and RAM latency,
not to mention the RAM price has skyrocketed these years\footnote{https://pcpartpicker.com/trends/price/memory/}.
ii) After loading $W_2$ in SIMD register, any data processing operation
on $W_2$ is wasting $5\times 32=160$ bits of computation power per cycle.

%------------the idea of using index for padding and what index to choose
%Given that the padding zeros are a big waste in ByteSlice,
%how can we fully leverage those empty space?
%\cbstart
%{\color{red}
%As a storage layout for main memory data processing,
%ByteSlice fails to utilize the limited
%memory space effectively due to those vacant bits.
%To make things worse, the memory price has doubled 
%over last 18 months\footnote{https://pcpartpicker.com/trends/price/memory/}.
%Therefore, it is crucial to fully leverage
%the vacant space in ByteSlice.
%}
%\cbend
Scan on ByteSlice is powerful by pruning lower-order 
{\em bytes} within segments.
However, it cannot skip a complete {\em segment}.
%due to its nature of {\em sequential} scan.
This may lead to contention of memory bandwidth when multi-threading is enabled\footnote{
%, which renders ByteSlice suffering from scalability issue
ByteSlice already consumes 98\% of the memory bandwidth with only 2 threads, thus becoming memory-bound.}.
%
%In order to sacrifice CPU time for aggressive data skipping, we propose to bring in 
%secondary index to fill up those padding zeros.
%A secondary index is a data skipping structure that aims at fetching relevant (thus less) data
%at the cost of additional CPU time for relevance checking,
Therefore, in this paper we propose to 
weave secondary index into the vacant bits (i.e., 
bits with padding zeros) of ByteSlice to enable data skipping.
%bring in secondary index to fill up those padding zeros.
In this way, we have chance to load less data into SIMD register, thus improving 
scan performance {\bf with zero space overhead}.
%Next, what index shall we use?
Basically, we want the index to be 
a) {\em lightweight} to fit within one segment,
and b) {\em size-adjustable} as columns have different code width (thus different number of padding zeros in each segment).
Therefore, we use a kind of non-dense bitmap index similar to 
Column Imprints~\cite{ColumnImprint} to pad up with 8-bit SIMD soft boundaries.

%----------Introduce DIFusion that enables skip-scan
In this paper, we propose a new main-memory storage layout 
coined \underline{D}ata \underline{I}ndex \underline{Fusion} (DIFusion)
that embeds secondary index into unused space of ByteSlice.
DIFusion enables {\em skip-scan} that allows data skipping during the sequential scan.
%that is different from 
%a sequential scan or a secondary index scan (e.g., probing through B$^{+}$-tree).
We illustrate skip-scan over DIFusion with the example in Figure~\ref{fig:difusion}a.
Skip-scan is performed segment-by-segment.
When $W_2$ is loaded into SIMD register during the scan of Segment 1, 
we could obtain a $5\times 32=160$-bit index (i.e., {\em index1}) {\bf in situ}.
%that replaces padding zeros when the DIFusion layout of this column is constructed.
Such index works as metadata that provides information about next few segment(s) to be scanned.
By scanning Segment 1,
we may be able to obtain the scan
results of Segment 1 as well as
get a notice to know ahead
what other segments (e.g., Segment 2 in Figure~\ref{fig:difusion}a) could be 
skipped.
%, say, Segment 2 for instance.
%We call Segment 2 the {\em indexing target} of {\em index1}.
%By examining {\em index1} and the filter predicate, 
%we have chance to obtain the scan results of Segment 2 without
%fetching it for processing.

To the best of our knowledge, this is the first work to enable data-skipping in in-memory code-packed data without any storage overhead.
The advantages of DIFusion are summarized as follows:
i) DIFusion fully exploits the memory bandwidth and computation power by
making {\em every bit} of the storage useful.
ii) DIFusion inherits the early stop capability from ByteSlice.
%iii) DIFusion enhances scan performance by bringing in secondary index with zero space overhead.
iii) DIFusion possesses the data-skipping ability of index with zero
space overhead.
It incurs extra index checking overhead indeed, but such overhead
is negligible to overlap with other instructions in the instruction
pipeline. By sacrificing insignificant CPU time for aggressive data skipping,
memory bandwidth contention is alleviated, especially in the case of
multi-threading.
%xu: robust issue removed ---not easy to understand?
%Such skipping ability has its greatest impact when the 
%column exhibits some degree of clustering[].
%or partial ordering
%Surprisingly, DIFusion remains robust even in the case of highly 
%unclustered data. The main reason is that, 
%the index checking overhead is so lightweight that overlaps
%with other instructions in the instruction pipeline.
%{\color{red}
%iv) DIFusion provides a single access path (i.e., skip-scan) that combines the advantages of both sequential scan and index scan, which frees the query optimizer from complex access path selection~\cite{stratos17aps}.
%}
%{\color{red}
%iv) authors in~\cite{stratos17aps} propose complex models to address the problem of access
%path selection, i.e., choosing between a sequential scan and a secondary
%index scan.
%DIFusion provides a single access path (i.e., skip-scan) that combines 
%the advantages of both sequential scan and index scan, 
%which alleviates the overhead of the database administrators or the tuning advisors.
%}
%v) sacrifice CPU time for skipping, address memory-bound issue 
% in the multi-threading case


%--------------what are the design options, i.e., challenges
It is challenging to design the optimal DIFusion layout for {\em each column},
as there are numerous design options that affect the scan performance.
For example, {\em in which byte should the index be positioned in each segment?}
%
%In Segment 1 of Figure 1b, the 160-bit index is scattered over the {\bf 2nd-byte} of the 32 codes (i.e, $W_2$).
%However, DIFusion has the chance to prune $W_2$ after scanning $W_1$ (because of early stop).
%If the pruning happens, the index in $W_2$ can never be retrieved, thus wasting its data skipping ability.
%As an alternative, we could {\em right shift five bits} for all codes (see Figure 1c),
%which enables us to put the index in the {\bf 1st-byte} (i.e., $W_1$).
%In this way, the index can definitely be accessed while scanning Segment 1.
%As a side effect, the early stop probability after scanning $W_1$ is reduced, since the code width for comparison in each byte of $W_1$ is reduced from 8-bit to 3-bit. 
ByteSlice right-pads zeros since it aims at maximizing the early stop probability.
If DIFusion still employs {\em padding-right} strategy, 
the index is always placed in the lowest-order byte.
In Segment 1 of Figure~\ref{fig:difusion}a, the 160-bit index is scattered over the {\bf 2nd-byte} of the 32 codes (i.e, $W_2$).
However, scan on DIFusion has the chance to prune $W_2$ after scanning $W_1$ (because of early stop).
If the pruning happens, the index in $W_2$ can never be retrieved, thus wasting its data skipping ability.
To this end, DIFusion also allows {\em left-padding} the index to the {\bf 1st-byte} (see Figure~\ref{fig:difusion}b).
%\cbstart
In that case, the index in $W_1$ can definitely be accessed, such that its indexing target (i.e.,
Segment 2) may be skipped by checking the index against the filter condition.
However, the early stop probability after scanning $W_1$ is lowered, since the number of bits for comparison in each byte of $W_1$ has been reduced from 8-bit to 3-bit.
%\cbend
%
Other factors like the size of each index make the design of DIFusion
even more complex.
We enumerate all design options, analytically quantify them, and come up with an {\em advisor}
to generate a satisfactory design for each column.
We conduct experimental evaluation on TPC-H, TPC-H Skew, SSB and real data.
Empirical results report a scan speedup of up to 2.1X, 2.3X, 2.1X, 2.8X on TPC-H,
TPC-H Skew, SSB, and real data, respectively.
%\cbstart
%{\color{red}   
%As an interesting observation from the experimental result,
%even with smallest space for indexing, 
%DIFusion yields much better performance than ByteSlice.
%It is worth noting that, scan on DIFusion yields much
%better performance than that on ByteSlice even for columns
%with only single vacant bit for the index.
It is worth noting that, scan on DIFusion is always no
worse than on ByteSlice,
even when a column has very few vacant bits left.
For instance, {\tt d\_yearmonthnum} column in SSB data  is encoded in $7$-bit.
Scan on this column still enjoys a speedup of 1.7X from DIFusion.
%\cbend
%}

% paper organization
The remainder of this paper is organized as follows: 
Section 2 presents some essential background information on ByteSlice and Column Imprints.
Section 3 presents our DIFusion storage layout.
Section 4 presents our advisor that recommends a design scheme for each column.
Section 5 presents the skip-scan algorithm over DIFusion.
Section 6 presents our experimental results.
Section 7 presents the related work.
Section 8 concludes our paper.



%these optimizations assume data in memory such that memory access is the bottleneck,
%but it requires large volume of memory


%what have been done to optimize memory usage, encoding?
%memory expensive
%Memory expensive and in limited capacity compared to data volume.
%Column values are encoded (for space).

==> relatedwork.tex <==
\section{Related Work}
In the past decade, the analytical market has been dominated by pure column-store systems like Vertica \cite{lamb2012vertica}, MonetDB/X100 \cite{monetdbx100}, and SAP HANA \cite{farber2012sap}. In current main-memory column store implementations like Vectorwise \cite{zukowski2012vectorwise} and SAP HANA, base column data by default are stored in standard data array \cite{monetdbx100}. Recently, the Bit-Packed storage layout \cite{willhalm2009simd, willhalm2013vectorizing} was proposed to store the base column data in a tightly bit-packed manner in memory. By doing so, the memory bandwidth usage can be reduced when scanning (filtering) the base data columns. Li and Patel \cite{li2013bitweaving} proposed the Vertical Bit Packing (VBP) and Horizontal Bit Packing (HBP) layouts, which store the base column data in a way that fully exploits the intra-cycle parallelism in modern processors to accelerate scans. 
ByteSlice \cite{feng2015} is a storage layout that chops data into multiple bytes and exploits early-stop capability by high-order bytes comparisons. 
It provides a single layout with which scans perform
better than on VBP and lookups perform as well as 
on HBP.
%and combines the advantages of both VBP and HBP without
%inheriting their disadvantages. 
However, ByteSlice and HBP waste much memory space for padding zeros. Although VBP does not waste any storage, scans and lookups on VBP are poorer than on ByteSlice \cite{feng2015}.
Our proposed DIFuion fully leverages the memory space by weaving a secondary index into
the vacant bits (i.e., bits originally padded with 0's).
It performs better than ByteSlice since it benefits from the data-skipping ability of index. 
%In current main-memory column store implementations, when an operator reads input produced from another operator, the input is assumed to be formatted as standard array
%\cite{kim2009sort, blanas2011design, blanas2013memory, balkensen2013hash, balkesen2013multi,
%shatdal1995adaptive, ross2007aggregate, ye2011scalable,
%inoue2007aa, chhugani2008efficient,
%ross2014comprehensive}.
%Under that implementation, after a lookup operation has retrieved a code from the base column, the code (together with its record number) is inserted into an array of, say, \texttt{struct~\{int32; int32;\}}. Subsequent operations like joins, aggregations and sorts would then take the array as inputs. Since these operators are not directly processing data straight from the base columns, their performances are independent of the storage layout of the base columns. Take sort as an example. Existing hardware-conscious sorting algorithms \cite{inoue2007aa, chhugani2008efficient, xu2016} also assume an array of \texttt{<SortKey, RecordID>} as input. When the sorting is carried out, the main concern is to exploit on-chip parallelism(e.g., SIMD) and to minimize cache misses and memory accesses.

In recent column-store implementations, instead of scanning the entire column, several state-of-the-art secondary indexes
\cite{Bitmap, bitmap2004vldb, BitMappedJoin, ColumnImprint}
are adopted to avoid accessing data that is certainly not part of the query result. Zonemap \cite{ColumnImprint} is a common choice for secondary index. A zonemap index notes the minimum and the maximum values found across a predefined number of consecutive values, called the zones. To evaluate a query using zonemaps, the minimum and maximum values of each zone are compared with the predicate of the query. If the
range of the predicate does not overlap with the range of a zone, the zone can be skipped simply. Bitmap \cite{Bitmap, bitmap2004vldb, BitMappedJoin} is another popular choice that works by mapping the column domain to bit vectors. Each vector has as many bits as the size of the column. For a value found in a specific position of the column, the corresponding bit in the mapping bit-vector is set. Deciding if a value satisfies a query involves first checking the corresponding bitmap, and returning only the position of the bits that are set. The checking is done with bitwise operators, making it cheaper to scan. Besides, Column Imprint \cite{ColumnImprint}
(also described in Section~\ref{sec:background}) is a cache conscious secondary index that empirically performs more effectively than zonemaps and bitmaps. Zonemaps, bitmaps and Column Imprints are efficient to skip data that is certainly not part of query result. However, all these methods, particularly bitmaps, cannot avoid using extra memory space especially in the case of large column cardinality and size. 
To the best of our knowledge, this is the first work to  embed the secondary index into the data storage,
such that the scan performance is enhanced without any storage overhead.



